MetaPrompting: Learning to Learn Better Prompts

Prompting method is regarded as one of the crucial progress for few-shot nature language processing. Recent research on prompting moves from discrete tokens based ``hard prompts'' to continuous ``soft prompts'', which employ learnable vectors as pseudo prompt tokens and achieve better performance. Though showing promising prospects, these soft-prompting methods are observed to rely heavily on good initialization to take effect. Unfortunately, obtaining a perfect initialization for soft prompts requires understanding of inner language models working and elaborate design, which is no easy task and has to restart from scratch for each new task. To remedy this, we propose a generalized soft prompting method called MetaPrompting, which adopts the well-recognized model-agnostic meta-learning algorithm to automatically find better prompt initialization that facilitates fast adaptation to new prompting tasks.Extensive experiments show MetaPrompting tackles soft prompt initialization problem and brings significant improvement on four different datasets (over 6 points improvement in accuracy for 1-shot setting), achieving new state-of-the-art performance.

==> 1.intro_backup2.0.tex <==
\section{Introduction}
Enabling models to learn from a few labeled examples, i.e., Few Shot Learning (FSL), is one of the key steps toward more human-like artificial intelligence. Recently, by taking advantage of large-scale Pretrained Language Models (PLM)~\cite{brown2020language}, prompting-based methods achieve impressive results for few-shot learning of Natural Language Processing (NLP)~\cite{gao2020making,liu2021makes,zhao2021calibrate}.

Prompting-based methods insert a piece of text, i.e. prompts, to the input examples, so that the few-shot task can be formulated as a (masked) language modeling problem. 
For example, say we want to classify the sentiment of the book review ``I will never read it again.'', we can append a prompt ``It was'' to the sentence, getting ``I will never read it again. It was''. It is natural to expect a higher probability from the PLM to generate ``terrible'' than ``great'' then. 
Such converting bridges the gap between pre-training and target tasks. Consequently, it has better transferability and less dependence on target task data.
% \atmasay{Rephrase this.}

\begin{figure}[t]
\centering
\begin{tikzpicture}
\draw (0,0 ) node[inner sep=0] {\includegraphics[width=0.9 \columnwidth, trim={0cm 0cm 0cm -1cm}, clip]{./figs/demo.png}};
\end{tikzpicture}
\caption{Comparison between the conventional soft-prompting method (left) and proposed MetaPrompting (right). 
$x$ denotes the query sentence, and $z$ denotes the learnable pseudo tokens within soft prompts. $\phi$ represents all trainable parameters. 
MetaPrompting exploits optimization-based meta-learning to find an initialization $\phi_\text{meta}$ that facilitates better and faster adaptation to new tasks.
\vspace*{-4mm}
% of which the embeddings are trainable. 
% \wxcomment{图中x和z不加粗}
%   $\phi$ represents all trainable parameters including soft prompt embeddings and LM parameters
% For trainable parameters of the soft-prompt model $\phi$, MetaPrompting exploits optimization-based meta-learning to find a task-general initialization $\phi'$ that facilitates fast adaptation to new tasks.
%  $\phi$ represents all trainable parameters for prompting based model soft prompt embeddings and LM parameters. \atmasay{Describe it in intro.}
}\label{fig:intro}
\end{figure}


The performance of prompting methods is found to be greatly affected by the design of prompts \cite{gao2020making}.
That is, a good prompt makes significant differences.
% , and it is necessary to search and optimize prompts.
Early attempts take manually-designed prompts and adopt automatic searching methods to optimize prompts. 
\citet{schick2020coling} and \cite{schick2021eacl} explore to automatically identify label words.
% \atmasay{Check this.}
In pursuit of better performance compared to hand-picked prompts, \citet{gao2020making} proposes LM-BFF to search both prompt templates and label words. 
AutoPrompt \cite{shin2020autoprompt} leverages gradient-based searching to find out the best prompts.
These prompts consist of discrete tokens, which limits the search space of prompts.
% Because it is not necessary to limit the prompt to human-interpretable natural language.
To further liberate the potential of prompts, recent works employ learnable vectors as prompt content and learn optimal prompts in continuous space, which is so-called ``soft prompts'' \cite{P-tuning,li2021prefix}.
Since they no longer require prompts to be composed of real words, these methods greatly expand the possibilities of prompts and thus achieve better performance \cite{liu2021pre}. 

However, despite the promising prospects of soft prompts, learning a good prompt is still far from trivial. 
Because soft-prompts search for optimal solutions in an infinite continuous space, the choice of the starting point for the search (i.e., prompt initialization) becomes crucial.
Soft-prompt is observed to be more sensitive to different initialization than discrete prompts in low data setting \cite{li2021prefix,liu2021pre}. 
Unfortunately, creating a perfect prompt initialization requires both understanding of LMs' inner workings and trial-and-error.
\citet{lester2021power} initialize soft prompt with the token embeddings of hand-crafted prompt directly.
\citet{zhong2021fact} search discrete tokens as better initialization, which show better performance.
What's worse is that these initializations are task-bounded.
Every time we confront a new task, the costly process for initialization design has to start from scratch.

In this paper, to tackle the above issues, we let loose the prompt design of a specific task, but instead focus on obtaining a task general prompt initialization that facilitates faster and better adaptation to new prompting tasks.
% We start by arguing that recent model-agnostic meta learning algorithms  (MAML \cite{MAML}) is a nice fit for the low-resource prompting task. Then, we proposed a generalized soft prompting algorithm called MetaPrompting based on the first-order version of  MAML \cite{Reptile} by viewing prompts in different label sets as separate meta prompting tasks (See Figure \ref{fig:intro}). 
% Following the essence of MAML, MetaPrompting allows learning to learn better initialization that can better adapt to unseen prompting scenarios.
% We dive deep into recently proposed optimization-based meta learning algorithms (MAML~\cite{MAML}, Reptile~\cite{Reptile} and etc.), to see if they can serve as a nice fit for low-resource prompting tasks. 

% Inspired by recently proposed optimization-based meta learning algorithms such as MAML~\cite{MAML}, Reptile~\cite{Reptile} and etc., we propose MetaPrompting, which is a generalized soft prompting algorithm based on optimization-based meta learning algorithms by viewing prompts in different label sets as separate meta prompting tasks (See Figure \ref{fig:intro}). 
% Following the essence of MAML, MetaPrompting allows learning to learn a better initialization for prompting model that can better adapt to unseen prompting tasks.
Recently proposed optimization-based meta learning algorithms, such as MAML~\cite{MAML}, Reptile~\cite{Reptile} and etc., aim at learning a parameter initialization point for better adaption. Following their essence, we propose MetaPrompting, which is a generalized soft prompting method powered by meta learning algorithms, to tackle soft prompt initialization problem. MetaPrompting learns general meta knowledge from source domain tasks to form a better soft prompt initialization, and thus adapts faster and better across various target domain tasks (See Figure \ref{fig:intro}). Extensive experiments show that MetaPrompting achieves promising performance with desired robustness. 
% A comparison between vanilla prompt tuning and MetaPrompting is illustrated in Figure \ref{fig:intro}. 


% On experiment of three different datasets, the proposed method achieves remarkable superiority over normally fine-tuned soft-prompt methods. 
% Besides, we also show that as a meta-learners, prompt-based models significantly outperform common meta-learners.

We summarize the main contribution of this paper as follows:

(1) We propose a novel prompting method MetaPrompting, which employs optimization-based meta learning algorithm to find adaptive initialization for soft-prompt methods. To the best of our knowledge, this is the first study of applying meta-learning to prompting problem setting.

(2) We conduct extensive experiments on three different datasets with various few-shot settings to evaluate MetaPrompting's performance. Results demonstrate the superiority of MetaPrompting over normally fine-tuned soft-prompt methods and SOTA meta-learning baselines.

(3) Further analysis experiments indicate that MetaPrompting significantly alleviates soft prompt initialization problem, and learns general meta knowledge from various source domains with desired robustness against prompt template variance.
We also study MetaPrompting's compatibility with different optimization-based meta learning methods and give empirical analysis of their performance difference.

All code and data will be publicly available.

==> 1_intro_backup1.0.tex <==
\section{Introduction}
Enabling model learn from a few labeled examples, i.e., Few Shot Learning (FSL), is one of the key step toward more human-like artificial intelligence. Recently, by taking advantage of large-scale Pretrained Language Models (PLM)~\cite{brown2020language}, prompting-based methods achieve impressive results for few-shot leaning of Natural Language Processing (NLP)~\cite{gao2020making,liu2021makes,zhao2021calibrate}.

Prompting-based method insert a piece of text, i.e. prompts, to the input examples, so that the few-shot task can be formulated as a (masked) language modeling problem. 
For example, say we want to classify the sentiment of the movie review "No reason to watch", we can append a prompt "It was" to the sentence, getting "No reason to watch. It was". It is natural to expect a higher probability from the LM to generate "terrible" than “great” then. 
Such converting can reduce the gap between pre-training and target task. Consequently, it has better transferability and less dependence on target task data.

Despite the great prospects and success, the performance of prompting methods are found to be greatly affected by the form of prompts \cite{}.
That is, a good prompt makes significant differences, and it is necessary to search and optimize prompts.
Early attempts to this issue adopt the search-based methods to find suitable tokens to form prompts. \cite{xxx},
Guo et al., 2021 show a soft Q-learning method that works well for prompt generation; AutoPrompt (Shin et al., 2020) proposes taking a gradient-based search (the idea was from Wallace et al., 2019, which aims for searching a universal adversarial trigger to make a model generate a specific prediction) to find out the best prompt for particular tasks.
All these prompt consist of discrete tokens, which limits the search prompts.
To beak the shackle of discrete space, later work used learnable vectors as prompt content and search optimal prompts with gradient, which is so called ``soft prompts''. 
Since they no longer require prompts to be composed of real words, these methods greatly expand the possibilities of prompts and thus achieve better performance. 

However, although gradient searching prompts in continue space liberates the potential of prompt, learning a good prompt is still far from trivial.
The performance of soft-prompts is tightly bound with the design of soft-prompting manner \cite{xxx}.
Previous work had to carefully design the soft prompt, including using anchor method that carefully pick which token to replace with
 soft prompts \cite{xxx}, and using adapter to embed soft-prompts into inner layers of PLM \cite{xxx}.
What further restricts its application is that most carefully modulated prompts are task specific.
Every time we confront to a new task, the costly prompt design process has to start from scratch.
% the carefully modulated prompt in the past will fail.

In this paper, to tackle the above issues, we let loose the specific prompt design, but instead focus on the learning of adaptive prompts. 
By introducing a meta-learning process to soft prompts, we propose \solution, which aims at learning to learn soft prompts that can better adapt to unseen tasks. 
On experiment of four different dataset, the proposed method achieves remarkable superiority over normally finetuned soft prompts methods. 
Besides, we also shows that as meta-learner, prompt based model significantly outperform common meta-learners.

The main contribution of this work is as following:
(1)
(2)
(3)

==> 2_related.tex <==
\section{Related Works}
In this section, we review related work in the fields of Language Model Prompting and Meta-learning. 
% \subsection{Pre-trained Language Models}
% The recent breakthrough in self-supervised~\cite{liu2020self} pre-trained language models has boosted the development of natural language processing.  GPT~\cite{radford2019language} first leverages the transformer architecture to pre-train on large-scale web texts. BERT~\cite{devlin2018bert} proposes the masked language modeling and creates the pre-train/fine-tuning paradigm. Later on, various kinds of language models grown up, including XLNet~\cite{yang2019xlnet} which innovates the permutation language modeling. RoBERTa~\cite{liu2019roberta} conducts detailed experiments to demonstrate useful techniques related to pre-training. BART~\cite{lewis2019bart}, T5~\cite{raffel2019exploring} and UniLM~\cite{dong2019unified} which try to unify the language understanding and generation.

% Pre-trained language models have had more than large impact on natural language processing, for they do not need much annotated data but perform self-supervised training on unlabeled data instead. As a result, pre-trained language models can make use of large unlabeled corpus to learn universal knowledge, and then be fine-tuned on downstream tasks to obtain better performance. Varying in training objectives and directionality of representation \cite{}, many pre-trained language models have achieved unprecedented performance on NLP tasks. Standard language models like GPT \cite{}, GPT2 \cite{}, GPT3 \cite{}, calculate each word's representation in a left-to-right order, and optimize the probability $P(\mathbf{x})$ of text from training corpus. Representative masked language models such as BERT \cite{} and ERNIE \cite{} compute bidirectional representation of each word, and are trained to restore the text from its corrupted version. 



\paragraph{Language Model Prompting}
% While the "Pre-train and Fine-tune" paradigm has become a conventional method to take advantage of the power of pre-trained language models in downstream tasks, models' performance may be limited because of the disparity between downstream tasks and those used for pre-training. To remedy this, prompting methods are proposed to better apply pre-trained language models to downstream tasks by aligning them with pre-training ones. 

Prompting methods are proposed to better apply pre-trained language models to downstream tasks by aligning them with pre-training tasks, and further explore the capability of pre-trained LMs. 

Early prompting method, GPT-3~\cite{brown2020language} and PET/iPET~\cite{PET} for example, uses hand-crafted prompt templates. Although promising results are achieved, the performance of these methods heavily relies on the selection of pre-defined prompt templates. However, hand-crafting prompt is extremely time-consuming, and hand-crafted prompts may be sub-optimal. 

A number of recent works focus on automating the search for better prompt templates. \citeauthor{shin2020autoprompt} propose AutoPrompt to search for better prompts based on gradient descent approach. \citeauthor{gao2020making} uses pre-trained T5 model to generate prompt templates for given sample text and answer words. Instead of searching for discrete template words, \citeauthor{li2021prefix} proposes prefix-tuning, where tokens with trainable continuous embeddings are placed at the beginning of the text to perform NLG tasks. P-tuning~\cite{P-tuning} also uses soft prompt, but inserts fixed anchor tokens and achieved promising results in NLU and knowledge probing tasks. In this work, we also combine soft prompt and anchor tokens as templates. Instead of directly applying the model in few-shot tasks, however, we adopt meta-learning methods to find a better initialization point for both soft prompt embeddings and MLM parameters, because they are very sensitive to initialization in few-shot settings~\cite{li2021prefix, liu2021pre}. 


\paragraph{Meta-Learning}
Meta-learning algorithms can be classified into metric-based methods, model-based methods and optimization-based methods. 
Metric-based methods such as Siamese Network \cite{koch2015siamese}, Matching Network \cite{vinyals2016matching} and Prototype Net \cite{PN}, are proposed to learn a metric space that gathers similar samples and separates distinct ones. 
The testing samples are mapped into the metric space, and their images are compared with those of training samples to make predictions. 
Model-based meta-learning algorithms use additional meta-learners to assist original learners to adapt faster to unseen tasks. The meta-learner can learn an optimization algorithm for the original leaner \cite{ravi2016optimization}, "memorize" training samples with memory-augmented neural networks \cite{graves2014neural}, or simply map training samples to activation states to assist model prediction \cite{mishra2017simple,qiao2018few}. 

However, metric-based methods require formulating tasks into specific forms, while model-based algorithms introduce additional architecture and parameters into the model. To this end, optimization-based methods like MAML~\cite{MAML} and Reptile~\cite{Reptile} are proposed to learn meta-knowledge in a model agnostic way. Specifically, these methods aim to find a better initialization point for model parameters, enabling the model to adapt faster to unseen tasks. 

==> 3_method_backup5.16.tex <==
\section{Method}
% Both prompting methods and optimization-based meta learning have shown promising results in few-shot learning tasks \cite{P-tuning,gao2020making,MAML}. 
% Since prompt-based methods, especially those adopting soft prompts, are very sensitive to parameter initialization~\cite{li2021prefix, liu2021pre}, we introduce optimization-based meta learning methods into prompting methods to find better initialization points for prompt-based models and further explore their capabilities in few-shot scenarios. 
In this section, we first introduce prompt-based model tuning methods in Section \ref{sec: 3.1}, and then describe how to construct Meta Prompting tasks in Section \ref{sec: 3.2}. 
Finally, we elaborate and formulate the Meta Prompting tuning objective and parameter updating strategies in Section \ref{sec: 3.3}. 

\begin{figure}[t]
 \centering
 \begin{tikzpicture}
 \draw (0,0 ) node[inner sep=0] {\includegraphics[width=0.9 \columnwidth, trim={1.6cm 15cm 7.5cm 1cm}, clip]{./figs/model.pdf}};
 \end{tikzpicture}
 \caption{
  An illustration of soft-prompting method. $x$ refers to the sample text, and $z$ represents soft prompt tokens. All trainable parameters are colored in blue, while fixed ones are colored in grey. 
 }\label{fig: model}
 \vspace*{-3mm}
\end{figure}

\subsection{Prompt-based Model Tuning}
\label{sec: 3.1}
% In Section \ref{sec: 2.1} we gave a description of how prompt-based methods work, and in this subsection, we show how to fine-tune the parameters of the prompt-based model. Following \cite{P-tuning}, we use soft-prompts with anchor tokens. To be specific, prompt tokens consist of soft tokens which are represented as trainable continuous embeddings as well as anchor tokens which are fixed as the embeddings of specific words. Hard-soft combined prompt templates render the model more flexible, while preserving enough semantic information to trigger the MLM to produce correct predictions.
% Similar with P-tuning(\cite{P-tuning}), we implement a 2-layer bi-directional LSTM network and a fully-connected transformation network on soft prompt embeddings, making it easier for prompt parameters to escape from local minima during training. 
% On the one hand, soft prompt tokens with trainable embeddings render the model more flexible, allowing it to adapt to downstream tasks more smoothly. On the other hand, fixed anchor tokens, ``\textit{?}'', ``\textit{topic}'' and etc. for instance, contain rich semantic information which could trigger MLM to produce correct predictions. 

% In Section \ref{sec: 2.1} we gave a description of how prompt-based methods work, and in this subsection, we show the way to fine-tune the parameters of the prompt-based model. 
In this work, we use soft-prompts with anchor tokens. As illustrated in Figure \ref{fig: model}, prompt tokens consist of soft tokens which are represented as trainable continuous embeddings (blue) as well as anchor tokens which are fixed as the embeddings of specific words (grey). Hard-soft combined prompt templates render the model more flexible, while preserving enough semantic information to trigger the MLM to produce correct predictions.
Similar with P-tuning(\cite{P-tuning}), we implement transformation layers on soft prompt embeddings, allowing them to escape from local minima more smoothly. 

% As illustrated in Figure \ref{fig: model}, we insert $z$, which indicates soft prompt tokens, into the prompt template. Embeddings of soft prompt tokens are continuous trainable parameters, and are colored blue in the figure. Note that we do not fix pre-trained MLM parameters in our model for better representation ability, because prompt-based methods with trainable MLM parameters have shown promising results over fine-tuning baselines~\cite{gao2020making, P-tuning}, while those with fixed MLM parameters struggle to over-perform the same baselines~\cite{shin2020autoprompt}. 
% As illustrated in Figure \ref{fig: model}, we insert $z$, which indicates soft prompt tokens, into the prompt template. During meta training, we do not fix pre-trained MLM parameters for better representation ability, because prompt-based methods with trainable MLM parameters have shown promising results over fine-tuning baselines~\cite{gao2020making, P-tuning}, while those with fixed MLM parameters struggle to over-perform the same baselines~\cite{shin2020autoprompt}. 

In this way, we define MLM parameters as $\theta$ and soft prompt token embeddings as $\phi$. Given a few-shot task $\tau$ where $\mathcal{D}_{\tau}=\{(\mathbf{x}_{i}, \mathbf{y}_{i})\}_{i\in\tau}$ represents training samples, the prompt tuning objective can be formulated as follows:
\vspace{-1mm}
\begin{equation}
\label{eq: adapt_obj}
\resizebox{.85\hsize}{!}{%
$\begin{split}
\theta^{*}, \phi^{*} &= \
\argmin\limits_{\theta, \phi}\mathcal{L}_{\mathcal{D}_{\tau}}(f_{\phi,\theta})\\
&=\argmax\limits_{\theta, \phi} \sum_{(\mathbf{x}_{i}, \mathbf{y}_{i})\in \mathcal{D}_{\tau}} \log P(\mathbf{y}_{i}|\mathbf{x}_{i}; \phi,\theta)
\end{split}$\quad,
}
\vspace{-1mm}
\end{equation}
where $\mathcal{L}$ is the loss function, and $f_{\phi,\theta}$ is prompt-based model parameterized by MLM parameters $\theta$ and soft prompt embeddings $\phi$. 

$\mathcal{D}_{\tau}$ contains few labeled data because of the high annotation cost in real-world scenarios. As a result, the initialization of parameters $\theta$ and $\phi$ are more than crucial to the model's performance. 
% In this work, we start prompt-based model tuning from meta-learned parameters $\theta_{meta}$ and $\phi_{meta}$, to alleviate soft prompt initialization problem. 




\subsection{Constructing Meta Prompting Tasks}
\label{sec: 3.2}
To get a better initialization point of parameters $\theta$ and $\phi$ that can easily adapt to new few-shot tasks, we propose to sample Meta Prompting tasks from accessible source data and fine-tune our model on these sampled tasks. This meta training process aims to simulate the model's adaption to new few-shot tasks. 

We sample each Meta Prompting task $\tau_{i}$ as follows: 
\vspace{-0.8mm}
\begin{equation}
\label{}
\tau_{i}=(\mathcal{D}_{\tau_{i}}^{support}, \mathcal{D}_{\tau_{i}}^{query})\text{,}
\vspace{-0.8mm}
\end{equation}
where $\mathcal{D}_{\tau_{i}}^{support}$ indicates the support set and $\mathcal{D}_{\tau_{i}}^{query}$ indicates the query set in traditional few-shot learning settings. 
Note that meta training tasks and meta testing tasks should be sampled from different domains, to prevent model from simply memorizing training samples.

% \subsection{Learning with  Meta Prompting Objectives}
\subsection{Applying Meta-learning to Prompting Models}
\label{sec: 3.3}
After constructing Meta Prompting tasks, we train our prompting model on these tasks to find a better initialization point. 
Figure \ref{fig: meta} illustrates the meta training and meta testing procedures of MetaPrompting. 
Given a Meta Prompting task $\tau_{i}$, we clone the model's parameters and simulate the adaption process of few-shot tasks by updating cloned model parameters $\theta_{i}^0$ and $\phi_{i}^0$ on $\mathcal{D}_{\tau_{i}}^{support}$. 
The adaption objective is given in Equation \eqref{eq: adapt_obj}, and this process can be formulated as: 
\vspace{-1.2mm}
\begin{equation}
\label{eq: adapt}
\resizebox{.85\hsize}{!}{%
$\begin{split}
&\theta^{k}_{i} = \theta^{k-1}_{i} - \alpha\nabla_{\theta^{k-1}_{i}}\mathcal{L}_{\mathcal{D}^{support}_{\tau_i}}(f_{\phi^{k-1}_{i},\theta^{k-1}_{i}}) \\
&\phi^{k}_{i} = \phi^{k-1}_{i} - \alpha\nabla_{\phi^{k-1}_{i}}\mathcal{L}_{\mathcal{D}^{support}_{\tau_i}}(f_{\phi^{k-1}_{i},\theta^{k-1}_{i}})
\end{split}$,
}
\vspace{-1.2mm}
\end{equation}
% \wxcomment{不需要花括号} 
where $\alpha$ indicates learning rate and $k=1, 2, 3, \dots$ indicates the inner step. 
% $\theta^{0}_{i}$ and $\phi^{0}_{i}$ represents cloned model parameters before adaption. 
% After adapting the cloned model on $\mathcal{D}_{\tau_{i}}^{support}$, we obtain an adapted model parameterized as $f_{\phi_{i},\theta_{i}}$. 
The goal of learning with Meta Prompting tasks is to minimize the loss of the adapted prompting model, which is parameterized as $f_{\phi_{i},\theta_{i}}$, on $\mathcal{D}_{\tau_{i}}^{query}$. This objective can be described as follows:
\vspace{-1mm}
\begin{equation}
\label{}
%\theta^{obj}_{i}, \phi^{obj}_{i} = \argmin\limits_{\theta_{i}, \phi_{i}} \mathcal{L}_{\mathcal{D}^{query}_{\tau_i}}(f_{\phi_{i},\theta_{i}}).
\theta^{obj}, \phi^{obj} = \argmin\limits_{\theta_{i}, \phi_{i}} \mathcal{L}_{\mathcal{D}^{query}_{\tau_i}}(f_{\phi_{i},\theta_{i}}).
\vspace{-1mm}
\end{equation}

% We point out that when  optimizing model parameters on $\mathcal{D}_{\tau_{i}}^{query}$, $f_{\phi_{i},\theta_{i}}$ are fixed. 

\begin{figure}[t]
 \centering
 \begin{tikzpicture}
 \draw (0,0 ) node[inner sep=0] {\includegraphics[width=0.97 \columnwidth, trim={1cm 10.5cm 8cm 1.3cm}, clip]{./figs/meta.pdf}};
 \end{tikzpicture}
 \caption{
  Meta training and testing procedures of MetaPrompting.
 }\label{fig: meta}
 \vspace*{-4mm}
\end{figure}


% Optimizing towards this objective is to mimic real few-shot text classification scenarios, and enable the model to find a better initialization point to adapt fast in new classification tasks. 
Optimizing towards this objective is to mimic real few-shot text classification scenarios, and enable prompting model to find a better initialization point for fast adaption in new classification tasks. 
Let $\beta$ be the learning rate when updating model parameters on $\mathcal{D}_{\tau_{i}}^{query}$, and $\mathbf{H}$ be Hessian matrix. 
% Given adapted prompt embedding parameters $\phi_{i}$ and pre-trained MLM parameters $\theta_{i}$, we formulate the second-order gradient of $\phi_{i}$  computed on $\mathcal{D}_{\tau_{i}}^{query}$ in the following form:
We formulate the second-order gradient of prompt parameter $\phi$  computed on $\mathcal{D}_{\tau_{i}}^{query}$ in the following form:
\vspace{-1.8mm}
\begin{equation}
\label{eq: MAML_update}
\begin{split}
\phi &\gets \phi - \beta \cdot g^{second}_{\phi}\\
&= \phi - \beta \nabla_{\phi} \mathcal{L}_{\mathcal{D}^{query}_{\tau_i}}(f_{\phi_{i},\theta_{i}})\\
&= \phi - \beta \nabla_{\phi_{i}} \mathcal{L}_{\mathcal{D}^{query}_{\tau_i}}(f_{\phi_{i},\theta_{i}}) \cdot \nabla_{\phi}(\phi_{i})\\
&= \phi - \beta \nabla_{\phi_{i}}\mathcal{L}_{\mathcal{D}^{query}_{\tau_i}}(f_{\phi_{i},\theta_{i}}) \cdot \\
&\qquad\quad(\mathbf{I} - \alpha\mathbf{H}_{\phi}(\mathcal{L}_{\mathcal{D}^{support}_{\tau_i}}(f_{\phi,\theta})) ),\\
\end{split}
\vspace{-4.5mm}
\end{equation}
% where we assume $\phi_{i}$ is $\phi$ adapted for single inner step on $\mathcal{D}^{support}_{\tau_i}$, and one Meta Prompting task is used for a parameter updating step. Pre-trained MLM parameters $\theta$ is updated in the same way as $\phi$ in Equation \eqref{eq: MAML_update}. 
where we assume $\phi_{i}$ is $\phi$ adapted for one inner step on $\mathcal{D}^{support}_{\tau_i}$. In practice, inner steps can be increased for better performance. Pre-trained MLM parameters $\theta$ is updated in the same way as prompt parameters $\phi$ in Equation \eqref{eq: MAML_update}.

% The calculation of second order gradient is extremely memory-consuming, especially when the model has large parameters. It can be well approximated by first order gradient \cite{MAML}, enabling the model to be trained with lower memory costs. In the first order form,  $\nabla_{\phi}(\phi_{i})$ is set as $\mathbf{I}$, ignoring the second order gradient term $\alpha\mathbf{H}_{\phi}(\mathcal{L}_{\mathcal{D}^{support}_{\tau_i}}(f_{\phi,\theta}))$. In this way, prompt token embedding parameters $\phi$ can be updated as follows:
% \vspace{-5mm}
% \begin{equation}
% \begin{split}
% \phi &\gets \phi - \beta \cdot g^{first}_{\phi}\\
% &= \phi - \beta \nabla_{\phi_{i}}\mathcal{L}_{\mathcal{D}^{query}_{\tau_i}}(f_{\phi_{i},\theta_{i}}) \cdot \mathbf{I}.
% \end{split}
% \label{eq: FOMAML_update}
% % \vspace{-12mm}
% \end{equation}
% \vspace{-3.4mm}

% Note that in this first-order approximation, second-order gradient terms may also appear, but they are not counted in the practical training process so they will not burden the training procedure. We refer to \cite{Reptile} for more details.\footnote{
% We adopt first-order approximation, because it brings limited performance changes (often less than $1.0$ accuracy) in experiments, but provides substantial improvements in speed and memory efficiency.}


\subsection{Stable and Memory-efficient Meta learning}
\label{sec: 3.4}

% Although broadly used in meta-learning tasks, MAML may suffer from training instability and thus cannot converge smoothly. To address this problem, we follow MAML++~\cite{antoniou2019train} to improve our model with Multi-Step Loss (MSL) and Per-Step Learning Rates (PSLR) tricks.
% MSL trick conduct loss back-propagation for each inner step during adapting. It alleviates the vanishing gradient problem in the stacked deep neural architecture constructed in adaption process. PSLR trick implements learnable learning rates for each inner step, to enable more flexible adaption on meta tasks. We do not include other MAML++ tricks into our model for their incompatibility or trivial performance improvement. 

% Although broadly used in meta-learning tasks, MAML suffers from training instability and thus cannot converge smoothly. To address this problem, we follow MAML++~\cite{antoniou2019train} to improve our model with Multi-Step Loss Back-propagation (MSLB).\footnote{We do not include other MAML++ tricks into our model for their incompatibility (BN layer tricks) or trivial performance improvement (Per-step adaption loss, cosine annealing learning rates).}
% MSLB conduct loss back-propagation for each inner step during adapting. 
% It alleviates the vanishing/exploding gradient problem in the stacked deep neural architecture constructed in adaption process. 
% As a result, the model behaves more stable during meta-training equipped with MSLB. 

Although broadly used in meta-learning tasks, MAML suffers from training instability and exploding memory consumption when model size and inner step grows. To address the first problem, we follow MAML++~\cite{antoniou2019train} to introduce Multi-Step Loss Back-propagation (MSLB) into prompting model tuning process.\footnote{We do not include other MAML++ tricks into our model for their incompatibility (BN layer tricks) or trivial performance improvement (Per-step adaption loss, cosine annealing learning rates).}
In this way, prompting model parameters receive optimization information from each inner step during adapting, alleviating the vanishing/exploding gradient problem in the stacked deep neural architecture constructed in adaption process. 
% As a result, the model behaves more stable during meta-training equipped with MSLB. 

As for the exploding memory consumption issue, we also explore to combine memory-efficient alternatives such as FOMAML~\cite{MAML} and Reptile~\cite{Reptile} with prompting model. FOMAML removes the high-order derivatives term in Equation~\ref{eq: MAML_update}, providing a cheap approximation for MAML. Reptile, on the other hand, updates model parameters towards the optimal point of each task, which is obtained by adapting the model on the support set samples. Equipped with these algorithms, MetaPrompting can learn meta knowledge to aid target domain tasks with limited memory consumption. 



==> 4_exp_backup.tex <==
\section{Experiment}
We conduct experiments by evaluating the proposed methods on three widely-used benchmark datasets with various low resource settings.

\subsection{Datasets}
Following previous works \cite{Few-shotTC,Frog-GNN}, we use the following three text classification datasets for experiments, which provide well-founded benchmarks for the meta-train \& meta-test setting and very in doamin and text length.
% We evaluate our method on the following three text classification datasets. 

\textbf{HuffPost headlines} contains around 200,000 news headlines from 2012 to 2018 obtained from HuffPost~\cite{HuffPost}. These headlines contain 41 categories, short and less grammatical, 
% and we sample 900 headlines for each category 
and the average text length is 13.04.

\textbf{Amazon product data} contains around 142.8 million product reviews from 1996 to 2014 from Amazon~\cite{Amazon}. These reviews contain 24 categories corresponding to their respective product categories, with very inconsistent length, 
% We sample 1000 reviews for each category, 
and their average length is 151.16.

\textbf{20 Newsgroups}~\cite{20News} contains 20 topics that are evenly distributed among 20,000 newsgroup documents,% each newsgroup corresponds to a topic~\cite{20News}. 
We used 20news-18828 version, 
% sample 941 news on average for each topic, 
same as~\cite{Few-shotTC}, and their average length is 285.13.

Regarding the categories selection of training, validation and testing sets, we use the same setting as~\citet{Few-shotTC}.
Also, we follow the same procedure to sample more tractable data subset from the original datasets.


\subsection{Implementation}
We use the pre-trained BERT (bert-base-uncased) with HuggingFaces codebase~\cite{wolf2019huggingface} as the pretrained language model.

For implements of soft prompting model, we adopt the same structure of \cite{P-tuning}, and use a two-layer biLSTM of 768 hidden units (same as the embedding size)  and MLP to calculate soft-prompt embeddings. 
We can divide the learnable parameters of entire prompting mmodel into two parts: pre-training model and prompt embedding. 
Except for the parameters \textit{bias} and \textit{LayerNorm.weight}, for the parameters of pre-training model, we use the weight decay wiht value of 0.1. We use AdamW~\cite{AdamW} to optimize two types of parameters, with initial learning rates of 1e-5 and 5e-5, respectively. And we use warmup method to update the learning rate.

Before meta-training stage, we generate 10000 training episodes, 2500 validation episodes and 7500 testing episodes comprehensively and randomly. During training stage, we train model with 100 sampled training episodes per epoch. When the when there is no validation loss decrease for 10 epochs, we apply early stopping. For testing, we test model on all 1000 test episodes, where we pick the best model according to performance on validation set. 
We set the batch size of all stages to 16.

% Regarding the categories selection of training, validation and testing sets, we use the same method as~\cite{Few-shotTC}. However, due to the particularity of our method, we set the labels to the same or similar natural language as the descriptive label of the original datasets. \atmasay{to label mapping}


\subsection{Baselines}
We compare our model (denoted as OUR) with following strong baselines:
% The following is a introduction for these baselines:

\textbf{1-NN} is a 1-nearest-neighbor classifier based on Euclidean distance.

\textbf{FineTune}~\cite{FT} is a method that obtains a larger model through pre-training, then fine-tunes (FT) the model through training samples (i.e. support set for few-shot learning) to fit the characteristics of dataset, and uses testing samples to evaluate the fine-tuning effect. 

\textbf{RR}~\cite{RR} is a classification method that adds L2 regularization on linear regression. For the neural network classifier, there may be inadequately training due to the small number of samples in the support set, and over-fitting phenomenon may occur because of the small support set. Therefore, the ridge regression (RR) that admits a closed-form solution is considered.


\textbf{MAML}~\cite{MAML} is a meta-learning method widely used in the field of few-shot learning, which meta-learns an initialization for the model to adapt to new tasks quickly by only a few gradient steps.

\textbf{Prototypical network}~\cite{PN}, a classic metric-based method, which is suitable for few-shot classification. It meta-learns a metric space by minimizing the Euclidean distance between the centroid of each category and the samples corresponding to these categories.

\textbf{DS}~\cite{Few-shotTC} is trained within a meta-learning framework to map the distribution signatures (DS) into attention scores for extracting more transferable features. It takes the diversity of language across tasks into account for text data, therefore can be applied to a wide variety of meta-learning methods.

Same as~\citet{Few-shotTC}, when comparing the above baselines, we compare the results based on three different representation methods AVG, IDF and CNN respectively, and give the optimal result of the corresponding datasets.

% 我先回宿舍了 (bohan
% OK

% sorry，解释上一段的作用的时候不小心点resolve找不回来了。
%上述的所有baseline的结果全部来自于DS这篇文章。但是DS对上面每个方法均给出了三种结果（因为有三种表示）
%这段的作用就是1.上述baseline的结果来自DS这篇文章；2.每个方法有三个结果，我们只比较他们的最大值。
%PS：这段适合加在实验细节还是实验结果还是这里？

\textbf{P-tuning}~\cite{P-tuning} is a prompt-based method that can combines prompt and MLM model to achieve a good few-shot learning effect by unifying the pre-training tasks and the downstream tasks that is converted into cloze. Different from the PET~\cite{PET}, P-tuning realizes the automatic construction of the prompt, turning the problem of construction into a continuous parameter optimization problem.

\textbf{Frog-GNN}~\cite{Frog-GNN} is a multi-perspective aggregation method based graph neural network for few-shot classification. Each query-support pair extracts more important characteristics of each category from neighbors with the help of the similarity between instance-level representations of graph nodes. 

\textbf{LaSAML}~\cite{LaSAML} is a meta-learning framework that focuses on mining the semantic information in the class-label and attaching it to the sentence as the input of the encoder to obtain discriminative sentence features . By implementing the framework with the prototypical network (i.e. LaSAML-PN),~\cite{LaSAML} achieve an improvement.

\textbf{KGML}~\cite{KGML} tries to bridge the gap between meta-training and meta-testing tasks by leveraging an external knowledge base, and to improve the generalization ability of the task, that is, to learn an additional representations for each sentence from the extracted sentence-specific knowledge graph. By combining with MAML (i.e. KGML-MAML) and prototypical network (i.e. KGML-PROTO) respectively, KGML demonstrates its role.

\textbf{DE}~\cite{DE} emphasizes the correlation between label representations to prevent possible label confusion in few-shot learning. Difference Extractor (DE) method can generate distinct label representations that embed information specific to each label. And like KGML, DE is also combined with MAML (i.e. DE-MAML) and prototypical network (i.e. DE-PROTO) to maximize its effect, and~\cite{DE} also gives the results of the combination of DE and MLMAN (i.e. DE-MLMAN,~\cite{MLMAN}).






\begin{table*}[t]
\small
% \setlength{\tabcolsep}{1.1pt}
\begin{tabular}{l cc cc cc cc}
\toprule
\multicolumn{1}{c}{Method} &
\multicolumn{2}{c}{20 News} &
\multicolumn{2}{c}{Amazon} &
\multicolumn{2}{c}{HuffPost} &
\multicolumn{2}{c}{Average}
\\
% \cmidrule(lr{0.5em}){1-2}
\cmidrule(lr{0.5em}){2-3}\cmidrule(lr{0.5em}){4-5}\cmidrule(lr{0.5em}){6-7}\cmidrule(lr{0.5em}){8-9}
 & 1 shot & 5 shot & 1 shot & 5 shot & 1 shot & 5 shot & 1 shot & 5 shot 
% & 1 shot & 5 shot & 1 shot & 5 shot & 1 shot & 5 shot 
\\
\midrule
\textsc{1-NN}       & $38.8$ &  $51.9$ & $51.4$ &  $67.1$ & $31.5$ &  $42.3$ & $ 40.5 $ &  $ 53.7 $ \\
\textsc{FineTune}        & $33.0$ &  $47.1$ & $45.7$ &  $63.9$ & $32.4$ &  $44.1$ & $ 37.0 $ &  $ 51.7 $ \\
\textsc{Proto}     & $37.8$ &  $46.5$ & $41.9$ &  $59.2$ & $34.8$ &  $50.2$ & $38.1  $ &  $ 51.9  $  \\
\textsc{MAML}      & $37.2$ & $48.6$ & $43.6$ & $62.4$ & $38.9$ & $53.7$ & $ 39.9 $ & $  54.9$  \\
\textsc{RR}        & $44.8$ &  $64.3$ & $60.2$ &  $79.7$ & $37.6$ &  $59.5$ & $ 47.5 $ &  $ 67.8$ \\
\textsc{DS} &  $52.1$ & $68.3$ & $62.6$ & $81.1$ & $43.0$ & $63.5$ & $ 52.5 $ & $ 70.9 $\\
\textsc{DE-MLMAN}        & $-$ &  $-$ & $-$ & $- $ & $49.7$ &  $60.9$ & $-$ &  $-$ \\
\textsc{DE-Proto}        & $-$ &  $-$ & $-$ & $- $ & $52.3$ &  $69.6$ & $-$ &  $-$ \\
\textsc{DE-MAML}         & $-$ &  $-$ & $-$ & $- $ & $51.8$ &  $67.3$ & $-$ &  $-$ \\
\textsc{KGML-Proto}        & $-$ &  $-$ & $58.6$ &  $74.5$ & $42.3$ &  $58.7$ & $-$ &  $-$ \\
\textsc{KGML-MAML}        & $-$ &  $-$ & $51.4$ &  $58.8$ & $44.2$ &  $54.1$ & $-$ &  $-$ \\
\textsc{LaSAML-PN}         & $-$ &  $-$ & $-$ & $- $ & $62.1$ &  $70.1$ & $-$ &  $-$ \\
\textsc{Frog-GNN}        & $-$ &  $-$ & $71.5$ &  $83.6$ & $54.1$ &  $69.6$ & $-$ &  $-$ \\
% add average version
% \textsc{DE-MLMAN}        & $-$ &  $-$ & $-$ & $- $ & $49.7$ &  $60.9$ & $ 49.7 $ &  $60.9 $ \\
% \textsc{DE-Proto}        & $-$ &  $-$ & $-$ & $- $ & $52.3$ &  $69.6$ & $ 52.3 $ &  $69.6 $ \\
% \textsc{DE-MAML}         & $-$ &  $-$ & $-$ & $- $ & $51.8$ &  $67.3$ & $ 51.8 $ &  $67.3 $ \\
% \textsc{KGML-Proto}        & $-$ &  $-$ & $58.6$ &  $74.5$ & $42.3$ &  $58.7$ & $ 50.4 $ &  $66.6 $ \\
% \textsc{KGML-MAML}        & $-$ &  $-$ & $51.4$ &  $58.8$ & $44.2$ &  $54.1$ & $ 47.8 $ &  $ 56.4$ \\
% \textsc{LaSAML-PN}         & $-$ &  $-$ & $-$ & $- $ & $62.1$ &  $70.1$ & $ 62.1 $ &  $ 70.1$ \\
% \textsc{Frog-GNN}        & $-$ &  $-$ & $71.5$ &  $83.6$ & $54.1$ &  $69.6$ & $  62.8$ &  $76.6 $ \\
\midrule
\textsc{P-Tuning}        & $52.1$ &  $59.4$ & $59.3$ &  $64.3$ & $49.1$ &  $65.9$ & $ 53.5 $ &  $63.2 $ \\
\textsc{Our} & $\bm{66.7}$  & $\bm{72.7}$ & $\bm{78.0}$ & $\bm{85.3}$ & $\bm{70.6}$ & $\bm{76.6}$ & $ \bm{71.7} $ & $\bm{78.2}  $\\
%\textsc{Our w/o FoMAML} & $\bm{65.2}$  & $\bm{69.6}$ & $\bm{72.6}$ & $\bm{78.1}$ & $\bm{67.9}$ & $\bm{72.9}$ & $ 68.5 $ & $ 73.5 $\\

\bottomrule
\end{tabular}
\centering
\caption{Results of 5-way 1-shot and 5-way 5-shot classification on three datasets.
The rows below the mid-line are prompting methods result. ‘-’ means that the result of this dataset is not given in the original paper.}
% \vspace{-5mm}
\end{table*}

\subsection{Main Results}
%List main results table and analysis here.

We evaluated P-tuning, and our method (OUR) in both 5-way 1-shot and 5-way 5-shot settings for all 3 datasets, and we report the best value that we can get from these methods on the validation set. These results are reported in Table 1. For other baseline that we will compare, if it provides the result for a certain dataset, we also choose the highest results of the corresponding dataset for comparison. All numbers in Table 1 are rounded down to one decimal place.

According to Table 1, Our model consistently achieve the best performance across all datasets. For 20 News dataset, our method improves 5-way 1-shot accuracy by 28.02\% and 5-way 5-shot accuracy by 6.44\%, against the best baseline. For Amazon dataset, our method improves 5-way 1-shot accuracy by 9.09\% and 5-way 1-shot accuracy by 2.03\%. And for HuffPost dataset, our method improves 5-way 1-shot accuracy by 13.68\% and 5-way 5-shot accuracy by 9.27\%. Meanwhile, we can get more conclusion from Table 1:

%\textbf{1.}When comparing against P-tuning and those simpler method, we can find that compared to a large number of dissimilar texts with different distributions (such as only using pre-trained model), the model can learn more useful knowledge from a large number of texts with the same distribution (such as episodes in other domains in the meta-training stage), although the model may have never seen the label of the text to be classified. 

\textbf{(1)} Comparing with P-tuning, we can see that our method has the advantage of using meta-learning to learn the better prompt, and that prompt can quickly adapt to new tasks. 

\textbf{(2)} Compared with simpler and more traditional methods such as FT, our method show the feasibility of using prompt for few-shot text classification tasks, and the prompt-based method is suitable for solving such NLP problems.

\textbf{(3)} Compared with the method based on prototype aggregation, the process of prototype aggregation may ignore a lot of useful support set information and the differences of samples from different categories. Because this method highlight the interaction in the same class and ignore inter-class relationship by simply encode support set samples of each class to prototype representations. But our method solves this problem because each episode contains more than one class.

\textbf{(4)} Compared with Frog-GNN, which achieves the best performance on Amazon dataset, our method has an improvement on the same dataset. Although it is unfair to compare with Frog-GNN for our method, because our method is inductive learning method, and Frog-GNN is transductive learning method, our method still achieves some higher scores.

\textbf{(5)} We can notice that our method has a greater improvement than DS on the 20news dataset, such as 1-shot our method can improve by about 14 points. This reflects that the advantages of using natural language labels to construct prompts, and the ability to use text and label information in few-shot learning scenario more deeply. And this advantage is more obvious on long text dataset such as 20news, because the bigger the text data, the larger the vocabulary and the amount of information it contains, the label and even the prompt we designed will have a closer connection with it.

\textbf{(6)} The difference between our method and the remaining methods, such as LaSAML method based on mining class label semantic information, DE method based on learning better label representation, our method shows that compared to focusing on how to make good use of the label itself (such as how to vectorize the labels better), the prompt-based method may become a new paradigm for solving downstream natural language processing problems.



%compare to MAML baselines is important indirect ablation of fix language model parameters. 


\begin{table}[t]
\small
% \setlength{\tabcolsep}{1.1pt}
\begin{tabular}{c cc cc}
\toprule
\multirow{2}{*}{Ada} &
\multicolumn{2}{c}{HuffPost} &
\multicolumn{2}{c}{Amazon} 
\\
% \cmidrule(lr{0.5em}){1-2}
\cmidrule(lr{0.5em}){2-3}\cmidrule(lr{0.5em}){4-5}
 & 1 shot & 5 shot & 1 shot & 5 shot
% & 1 shot & 5 shot & 1 shot & 5 shot & 1 shot & 5 shot 
\\
\midrule
\textsc{3}       & $68.8$ &  $73.1$ & $70.8$ &  $77.0$  \\
\textsc{5}       & $69.4$ &  $73.4$ & $72.1$ &  $79.9$\\
\textsc{10}     & $70.6$ &  $75.7$ & $77.1$ &  $83.4$\\
\textsc{15}     & $70.4$ &  $76.6$ & $78.0$ &  $85.3$    \\

\bottomrule
\end{tabular}
\centering
\caption{
Effects of adaptation step number (ada) on HuffPost and Amazon.
}
% \vspace{-5mm}
\end{table}


\begin{table}[t]
\small
% \setlength{\tabcolsep}{1.1pt}
\begin{tabular}{l cc cc}
\toprule
\multirow{2}{*}{Method} &
\multicolumn{2}{c}{HuffPost} &
\multicolumn{2}{c}{Amazon} 
\\
% \cmidrule(lr{0.5em}){1-2}
\cmidrule(lr{0.5em}){2-3}\cmidrule(lr{0.5em}){4-5}
 & 1 shot & 5 shot & 1 shot & 5 shot
% & 1 shot & 5 shot & 1 shot & 5 shot & 1 shot & 5 shot 
\\
\midrule
\textsc{Our}       & $70.6$ &  $76.6$ & $78.0$ &  $85.3$  \\
{w/o first order approx}       & $70.2$ &  $75.6$ & $75.1$ &  $83.7$\\
{w/o meta-learning}       & $67.9$ &  $72.9$ & $72.6$ &  $78.1$\\


\bottomrule
\end{tabular}
\centering
\caption{
Ablation analysis on meta learning process.
}
% \vspace{-5mm}
\end{table}


% \begin{table}[t]
% % \small
% % \setlength{\tabcolsep}{1.1pt}
% \begin{tabular}{c cc cc cc cc}
% \toprule
% \multirow{2}{*}{No.} &
% \multicolumn{2}{c}{Prompt} 
% \\
% \midrule
% \textsc{1}       & [TEXT], the topic is [MASK] (~\textit{original}) &   \\
% \textsc{2}       &  [MASK] is the topic of [TEXT] &  \\
% \textsc{3}       & What is the topic of [TEXT]? [MASK] & \\


% \bottomrule
% \end{tabular}
% \centering
% \caption{
% pad
% }
% % \vspace{-5mm}
% \end{table}

\begin{table}[t]
\small
% \setlength{\tabcolsep}{1.1pt}
\begin{tabular}{c cc cc cc cc}
\toprule
\multirow{2}{*}{Method} &
\multicolumn{2}{c}{HuffPost} &
\multicolumn{2}{c}{Amazon} 
\\
% \cmidrule(lr{0.5em}){1-2}
%\cmidrule(lr{0.5em}){2-3}\cmidrule(lr{0.5em}){4-5}\cmidrule(lr{0.5em}){6-7}\cmidrule(lr{0.5em}){8-9}
& 1 shot & 5 shot & 1 shot & 5 shot
% & 1 shot & 5 shot & 1 shot & 5 shot & 1 shot & 5 shot 
\\
\midrule
\textsc{P-tuning}       &  $\pm{4.53}$ &  $\pm{3.66}$  \\
\textsc{OUR}       & $\pm{1.00}$ & $\pm{0.11}$\\
% \textsc{P-tuning}       & $45.1$ &  $\pm{4.53}$ & $54.4$ &  $\pm{3.66}$  \\
% \textsc{OUR}       & $68.9$ &  $\pm{1.00}$ & $73.2$ &  $\pm{0.11}$\\
\bottomrule
\end{tabular}
\centering
\caption{
Analysis for anti-disturbance against changing of prompting form. \atmasay{Describe the prompts in line.}
}
% \vspace{-5mm}
\end{table}


\subsection{Analysis}

\paragraph{Analysis on Prompt Learning}

By observing the changes of the different methods loss in the meta-testing stage, we can get more information about prompt-learning.

We select 5-way 5-shot to get the best model on Amazon dataset to draw loss changing curve in the meta-testing stage. Specifically, we randomly sample 20 numbers from 1000 numbers as the location where we can choose testing episodes, then sample specific testing episodes according to the numbers, and then output loss after fine-tuning the best model.

According to Figure 4, the convergence speed of our method loss is the fastest, while the P-tuning without any additional relevant text has a slower convergence speed, and the convergence quality is much lower than the other two methods. We will also find that out method is better than Pre-train P-tuning method in term of both convergence speed and quality (although there is a small amount of overlap). This show the role of meta-learning for prompt-learning. 

\begin{figure}[t]
 \centering
 
 \begin{tikzpicture}
 \draw (0,0 ) node[inner sep=0] {\includegraphics[width=0.97 \columnwidth, trim={0.2cm 0.1cm 0.4cm 1cm}, clip]{./figs/loss.png}};
 \end{tikzpicture}
 \caption{
  Analysis on prompt learning. 
 }\label{fig:project_dim}
\end{figure}


\paragraph{Anti-disturbance analysis}

Table 4 shows the different prompt structures used in this paper, the ~\textit{original} prompt produced all the results of this paper except this section. Specifically, we use HuffPost dataset with 3 adaptation step number. In addition to the original prompt, we follow the order of disrupting [TASK], [MASK] and keywords (such as \textit{topic}), using declarative sentence and interrogative sentences to construct prompts.

From Table 5, we can learn that with the changing of prompt, our method has better stability than P-tuning. Especially 5-way 5-shot, our method controls the standard deviation at $\pm{0.11}$. Table 5 shows that using meta-learning, our method can learn a more stable and accurate prompt, which can be transferred to new tasks faster, and reflects good anti-disturbance ability.

\paragraph{Adaptation step number analysis}%???
According to Table 2, we find that whether it is 5-way 1-shot or 5-way 5-shot, as the adaptation step number (ada) increases, the effect of our method usually also increases. For the consideration of training efficiency, we directly selected 3, 5, 10, and 15 to carry out our experiment and chose the best result of them. And we knows that our method needs to be more patient, more refined, and softer to extract text features, there may be a better ada that can make the results better.


\paragraph{Analysis on meta-learning method}

Through Table 1, we see that our FOMAML-based meta-learning method has a very good ability on the few-shot text classification task. In this section, we explore the impact of replacing FOMAML with MAML, or even abandoning meta-learning method (i.e. only using pre-trained models for fine-tuning) on few-shot text classification tasks.

Compared with P-tuning method based on the pre-training model (i.e. OUR w/o META-LEARNING), we believe that the reason why our method is better is that the meta-learning method we use can better learn the features of the texts, especially in few-shot learning, the advantage of our method are more obvious, and the knowledge from the source domain can be transferred to the new tasks more quickly. Compared with the method that only based on pre-training or other methods, we find that the method based on meta-learning is more refined, softer and more essential in learning features.

By comparing with the method using MAML (OUR w/o FIRST ORDER APPROX), we can observe that the results of them are roughly similar, and the difference is not very big. This is because FOMAML is only a first order gradient approximation of MAML, and the algorithm of them are almost the same. However, because MAML uses second order gradient to meta-learn, the video memory growth of MAML is exponential to FOMAML. Therefore, compared with our method, it may not be faster to apply the model generated in meta-training stage to new tasks (i.e. MAML-based methods may require a larger adaptation step number compared to FOMAML-based methods). Therefore, considering training efficiency and video memory size, we choose FOMAML.





% \begin{table}[t]
% 	\centering
% 	\footnotesize
%     % \small
% 	\begin{tabular}{lcccc}\toprule
% 		\multirow{2}{*}{\textbf{disturbance}} &
% 		\multicolumn{2}{c}{\textbf{Seed}} & 
% 		\multicolumn{2}{c}{\textbf{Prompt}} 
% 		\cmidrule(lr{0.5em}){2-3}\cmidrule(lr{0.5em}){4-5}
% 		\\
		
% 		\midrule
%         % {Sequence Labeling BERT}  & 6.46 &    \\
%         % {EntLM} & 6.64 & \\
%         % \hdashline
%         % {NNShot}  & 15.98 &    \\
%         % {StructShot}  & 17.66 &   \\
%         % \hdashline
%         % {Template-based BART}  & 408.0 &  236.0  \\
%         % {Baseline (Forward Prompt)}  & 408.0 &  236.0  \\
%         \textsc{P-Tuning}  &  &  \\
% 		\textsc{Ours}   &  &  \\
% 		\bottomrule
% 	\end{tabular}
% 	\caption{ 
% % 	\footnotesize 
% 		Stability analysis of prompt initialization.
% 	}\label{tbl:5shot}
% % 	\vspace*{-4mm}
% \end{table}




==> 6_background_backup1.0.tex <==
% \section{Related Works}
% In this section, we review related work in the fields of Language Model Prompting and Meta learning. 

% \paragraph{Language Model Prompting}
% Prompting methods are proposed to better apply pre-trained language models to downstream tasks by aligning them with pre-training tasks, and further explore the capability of pre-trained LMs. 

% Early prompting method, GPT-3~\cite{brown2020language} and PET/iPET~\cite{PET} for example, uses hand-crafted prompt templates. Although promising results are achieved, the performance of these methods heavily relies on the selection of pre-defined prompt templates. However, hand-crafting prompt is extremely time-consuming, and hand-crafted prompts may be sub-optimal. 

% A number of recent works focus on automating the search for better prompt templates. \citeauthor{shin2020autoprompt} propose AutoPrompt to search for better prompts based on gradient descent approach. \citeauthor{gao2020making} uses pre-trained T5 model to generate prompt templates for given sample text and answer words. Instead of searching for discrete template words, \citeauthor{li2021prefix} proposes prefix-tuning, where tokens with trainable continuous embeddings are placed at the beginning of the text to perform NLG tasks. P-tuning~\cite{P-tuning} also uses soft prompt, but insert fixed anchor tokens and achieved promising results in NLU and knowledge probing tasks. In this work, we also combine soft prompt and anchor tokens as templates. Instead of directly applying the model in few-shot tasks, however, we adopt meta learning methods to find a better initialization point for both soft prompt embeddings and MLM parameters, based on the fact that are very sensitive to initialization in few-shot settings~\cite{li2021prefix, liu2021pre}. 


% \paragraph{Meta Learning}
% Meta learning algorithms can be classified into metric-based methods, model-based methods and optimization-based methods. 
% Metric-based methods such as Siamese Network \cite{koch2015siamese}, Matching Network \cite{vinyals2016matching} and Prototype Net \cite{PN}, are proposed to learn a metric space that gathers similar samples and separates distinct ones. 
% The testing samples are mapped into the metric space, and their images are compared with those of training samples to make predictions. 
% Model-based meta learning algorithms use additional meta learners to assist original learners to adapt faster to unseen tasks. The meta learner can learn an optimization algorithm for the original leaner \cite{ravi2016optimization}, "memorize" training samples with memory-augmented neural networks \cite{graves2014neural}, or simply map training samples to activation states to assist model prediction \cite{mishra2017simple,qiao2018few}. 

% However, metric-based methods require formulating tasks into specific forms, while model-based algorithms introduce additional architecture and parameters into the model. To this end, optimization-based methods like MAML~\cite{MAML} and Reptile~\cite{Reptile} are proposed to learn meta knowledge in a model agnostic way. Specifically, these methods aim to find a better initialization point for model parameters, enabling the model to adapt faster in unseen tasks. 

\section{Preliminaries and Related Works}
% In this section, we introduce the basis of prompt-based methods and meta learning algorithms. We elaborate the procedure of prompting language models in Section \ref{sec: 2.1}, and briefly describe the commonly used meta learning algorithms. 
In this section, we review related work and provide preliminaries about Language Model Prompting and Meta learning. 
\subsection{Prompting Language Models}
\label{sec: 2.1}
Prompting methods are proposed to better apply pre-trained language models to downstream tasks by aligning them with pre-training tasks, and further explore the capability of pre-trained LMs. For Masked Language Models (MLMs), the first step is to convert a sample text $x$ to $x_{prompt}$ by inserting prompt words which contain \texttt{[MASK]} tokens. Taking the news headline classification task as an example, the prompted text is given as:
\vspace{-1mm}
\begin{equation}
\label{eq:lm-classification}
\resizebox{.85\hsize}{!}{%
$x_{prompt} = \text{\texttt{[CLS]}~$x$~{The topic is}~\texttt{[MASK]}~. \texttt{[SEP]}}$,
}
\vspace{-1mm}
\end{equation}
where ``The topic is [MASK]'' are prompt tokens. Then, we task pre-trained MLM to complete the prompted text $x_{prompt}$, and the word to be filled at \texttt{[MASK]} position is regarded as an answer. An answer-label map is then used to convert the word probability distribution at \texttt{[MASK]} to classification results. 
% For news headline classification task, answer `arts' and `culture' can be mapped to label `ARTS \& CULTURE', while `environment' can be mapped to label `ENVIRONMENT'. 
The average probability of each label's corresponding answers is computed as the label's final probability.

Early prompting methods, such as GPT-3~\cite{brown2020language} and PET/iPET~\cite{PET}, use hand-crafted prompt templates. Although promising results are achieved, the performance of these methods heavily relies on the selection of pre-defined prompt templates. Moreover, designing prompts is extremely time-consuming, and hand-crafted prompts may be sub-optimal. 

A number of recent works focus on automating the search for better prompt templates. \citeauthor{shin2020autoprompt} propose AutoPrompt to search for better prompts based on gradient descent approach. \citeauthor{gao2020making} uses pre-trained T5 model to generate prompt templates for given sample text and answer words. Instead of searching for discrete template words, \citeauthor{li2021prefix} proposes prefix-tuning, where tokens with trainable continuous embeddings are appended at the beginning of the text to perform NLG tasks. P-tuning~\cite{P-tuning} also uses soft prompt, but insert fixed anchor tokens and achieved promising results in NLU and knowledge probing tasks. In this work, we also combine soft prompt and anchor tokens as templates. Instead of directly applying the model in few-shot tasks, however, we adopt meta learning methods to find a better initialization point for both soft prompt embeddings and MLM parameters, based on the fact that are very sensitive to initialization in few-shot settings~\cite{li2021prefix, liu2021pre}.
Note that a recent work meta-tuning~\cite{zhong2021adapting} also conduct meta learning on a number of source domain tasks, but their method consumes heavy human labor to design hard prompts for each task. 

% \paragraph{Multi-mask prompt.} Above we discussed how to reformulate an NLP task with prompt methods, where each prompted input only contains one single \texttt{[MASK]}. However, answers can be more complicated and will be tokenized into multiple word pieces. As a result, multiple \texttt{[MASK]} tokens should present in $x_{prompt}$ to enable $\mathcal{L}$ to make predictions for these answers. To compute the probability of answers which take up multiple \texttt{[MASK]} positions, we follow PET \cite{PET}. During training stage, the probability of answer $y$'s word pieces at \texttt{[MASK]} positions is computed in a single forward pass, and the probability of answer $y$ is given as: 
% \begin{equation}
% \label{eq:lm-classification}
% \resizebox{.85\hsize}{!}{%
% $q_{train}(y|x_{prompt}) = \prod_{i=1}^{k}q^{i}(y_{i}|x_{prompt})$,
% }
% \end{equation}
% where $y_{i}$ is the $i$th word piece of answer $y$, and $q^{i}(y_{i}|x_{prompt})$ represents the probability of $y_{i}$ to be filled in the $i$th \texttt{[MASK]} of $x_{prompt}$. 

% The probability of each answer is computed in a single pass for efficiency in the training stage. During evaluation stage, the probability is computed in a different way. $q_{eval}(y|x_{prompt})$ is computed as \cite{PET}: 
% \begin{equation}
% \label{eq:lm-classification}
% \resizebox{.85\hsize}{!}{%
% $q_{eval}(y|x_{prompt}) = 
% \begin{cases}
% 1& \text{if $k$=0}\\
% q^{j}(y_{j}|x_{prompt})*q_{eval}(y^{\prime}|x_{prompt}^{\prime})& \text{if $k$>0}
% \end{cases}$,
% }
% \end{equation}
% where $q^{j}(y_{j}|x_{prompt})=\max \limits_{i}q^{i}(y_{i}|x_{prompt})$. $x_{prompt}^{\prime}$ is $x_{prompt}$ filled with $y_{j}$ at the $j$th \texttt{[MASK]} position and $y^{\prime}$ is $y$ except $y_{j}$. Note that although described as probabilities, both $q_{train}$ and $q_{eval}$ are not normalized probabilities where the sum equals to 1. A \rm{Softmax} function is used to tackle with it. 


\subsection{Meta Learning}
% Meta learning, also known as ``learning to learn", has been drawing more interest in recent years for its remarkable capability in tackling conventional challenges such as data quantity limitation and computation resource limitation. A fundamental objective of meta learning is enabling the model to adapt better and faster to new and limited data in different tasks. 

% To this end, optimization-based meta learning methods propose to optimize model parameters to find a golden initialization point, so that the model can adapt faster and achieve better performance in unseen tasks, even only given limited data quantity and computation resources. MAML \cite{MAML} and Reptile \cite{Reptile} are representative optimization-based meta learning algorithms, which optimize the parameters in a model-agnostic way. 
% In these methods, models are trained on few-shot episodes to learn to adapt faster in low-resource tasks. The training objective is set to find a better parameter initialization point, with which the model can adapt to unseen tasks more smoothly. 



Meta learning algorithms can be classified into metric-based methods, model-based methods and optimization-based methods. 
Metric-based methods such as Siamese Network \cite{koch2015siamese}, Matching Network \cite{vinyals2016matching} and Prototype Net \cite{PN}, are proposed to learn a metric space that gathers similar samples and separates distinct ones. 
The testing samples are mapped into the metric space, and their images are compared with those of training samples to make predictions. 
Model-based meta learning algorithms use additional meta learners to assist original learners to adapt faster to unseen tasks. The meta learner can learn an optimization algorithm for the original leaner \cite{Ravi2017OptimizationAA}, "memorize" training samples with memory-augmented neural networks \cite{graves2014neural}, or simply map training samples to activation states to assist model prediction \cite{mishra2017simple,qiao2018few}. 

However, metric-based methods require formulating tasks into specific forms, while model-based algorithms introduce additional architecture and parameters into the model. 
To this end, optimization-based meta learning methods are proposed to improve model's optimization procedure. 
\citeauthor{Andrychowicz2016LearningTL} and \citeauthor{Ravi2017OptimizationAA} train recurrent neural networks to transform vanilla gradient descent direction to for better optimization results.  
MAML~\cite{MAML} optimizes model parameters to find a better initialization point, so that the model can adapt faster and achieve better performance in unseen tasks. In addition to MAML, more elaborate methods also learns inner step gradient descent direction~\cite{li2017meta} and inner step sizes~\cite{antoniou2019train}. Utilizing first-order derivatives, FOMAML~\cite{MAML} and Reptile \cite{Reptile} are proposed to reduce the memory consumption of high-order derivative calculation. 


% In these methods, models are trained on few-shot episodes to learn to adapt faster in low-resource tasks. The training objective is set to find a better parameter initialization point, with which the model can adapt to unseen tasks more smoothly. 
% To this end, optimization-based methods like MAML~\cite{MAML} and Reptile~\cite{Reptile} are proposed to learn meta knowledge in a model agnostic way. Specifically, these methods aim to find a better initialization point for model parameters, enabling the model to adapt faster in unseen tasks. 


%\texttt{}
%\text{\rm Softmax}
%\textsc{Softmax}
%\bm{}
%\paragraph{Metric learning. }
%\paragraph{Model-based methods. }
%\paragraph{Optimization-based methods. }
%nice fit to the low-resource; prompting  task






























==> pt/pt_LAMA.tex <==
\hide{
\begin{subtable}
    \centering
    \begin{tabular}{p{1.3cm}<{\centering}|p{2.6cm}<{\raggedright}|c|c|c|c}
        \toprule[1pt]
        Prompt type                 & Model                                 & 1-1   & N-1   & N-M   & Total \\ \hline
        \multirow{3}*{\makecell[c]{Original\\(MP)}} & BERT-base                             & 67.8  & 30.4  & 23.3  & 31.1 \\ 
        ~                           & BERT-large                            & 74.5  & 34.2  & 24.3  & 32.3 \\ 
        ~                           & E-BERT                                & -     & -     & -     & 36.2 \\ \hline
        \multirow{3}*{Discrete}     & LPAQA \tiny{(BERT-base)}              & -     & -     & -     & 34.1 \\
        ~                           & LPAQA \tiny{(BERT-large)}             & -     & -     & -     & 39.4 \\
        ~                           & AutoPrompt \tiny{(BERT-base)}         & -     & -     & -     & \underline{43.3} \\ \hline
        \multirow{2}*{\solution}    & BERT-base                             & 59.6  & 53.3  & 38.4  & 48.3 \\
        ~                           & BERT-large                            & 63.2  & 56.1  & 41.9  & \textbf{50.6} \\
        \toprule[1pt]
    \end{tabular}
\end{subtable}%
}



\subsection{Knowledge Probing}
Knowledge probing, or referred to as fact retrieval, evaluates how much real-world knowledge has language models gained from pre-training. The LAMA~\cite{petroni2019language} dataset evaluates it with cloze tests created from triples selected in the knowledge bases. For example, we will transform the triple (Dante, born-in, Florence) into a cloze sentence with the handcraft prompt ``Dante was born in [MASK].", and then we ask language models to inference the target. Because we want to evaluate knowledge gained from pre-training, pre-trained language models' parameters are fixed (i.e., not fine-tuned).

\subsubsection{Datasets and Formulation}
\vpara{Datasets.} 
LAMA enforces all answers in single-token format. We first adopt the original LAMA-TREx dataset, consisting of 41 Wikidata relations and altogether 34,039 testing triples (namely LAMA-34k, which covers all BERT vocabularies). Because GPT and BERT's vocabularies are different, we set up another version of LAMA, which covers the intersection of GPT and BERT's vocabulary. This subset adds up to about 29,000 testing triples, and we name it the LAMA-29k.

As for training, all prompt searching approaches need some additional data to train or find the prompts. We follow the setting in AutoPrompt~\cite{shin2020autoprompt}, where the authors construct a training set from the original TRE-x dataset. This training set is similar to the test set but with a slightly different answer distribution.

\vpara{Evaluation.} 
Originally, LAMA has provided a handcraft prompt for each relation such as Table \ref{tab:motivation_lama}, which are effective but sub-optimal. For bidirectional masked language models, we only need to replace the ``[X]" with the subject entity and ``[Y]" with the [MASK] token; for unidirectional language models such as GPT, following LAMA's original setting on Transformer-XL~\cite{dai2019transformer}, we use the network output just before the target position. In terms of conducting \solution, we use a (3, sub,3, obj,3) template for bidirectional models and (3, sub,3, obj) for unidirectional models, where the number indicates the number of prompt tokens. In this knowledge probing task, we do not use any anchor tokens. During the training, we set the learning rate to 1e-5 and use the Adam optimizer.

\subsubsection{Results}
\vpara{General performance.}
The results are presented in Table \ref{tab:lama_results}. The \solution significantly pushes the boundary of knowledge probing from 43.3\% to 50.6\% in LAMA-34k and 45.2\% to a maximum of 64.2\% in LAMA-29k. This result strongly suggests that language models capture far more knowledge than people previously believed by merely finding a better prompt and without fine-tuning. When \solution is compared with previous discrete prompt searching approaches such as AutoPrompt~\cite{shin2020autoprompt} and LPAQA~\cite{jiang2020can} on the same-size models, \solution still outperforms them.

\vpara{\solution v.s. Fine-tuning.}
It is not allowed to change the pre-trained model's parameters by fine-tuning in traditional knowledge probing. We seek to evaluate how much knowledge has language models learned during pre-training. However, this work's essential aspect is to compare \solution and fine-tuning, particularly on unidirectional language models like GPT. We are especially interested in the following question: Are unidirectional and bidirectional language models gaining similar improvement from \solution?

To make a comprehensive review on existing tuning methods, we include the following approaches: 1) Manual Prompt (MP): use original handcraft prompts from LAMA. 2) Fine-tuning (FT): only to present the subject and fine-tune the model to predict the object. 3) Manual Prompt with Fine-tuning (MP+FT): fine-tuning the language model with the handcraft prompts. 4) \solution: use continuous prompts (while fixing language models' parameters).

We implement the four strategies in the LAMA-29k (see Table \ref{tab:lama_results}, right), and we find that \solution is comparable to or better than fine-tuning-based methods, which is surprising but reasonable. The surprising thing is that fine-tuning should have been more potent since it tunes all language models' parameters, while \solution not. However, it is also reasonable because, in terms of knowledge probing, many facts can only be hard-coded rather than inferenced by language models. The fine-tuning of parameters might result in catastrophic forgetting. On the contrary, \solution does not change the pre-trained models' parameters but evoke the stored knowledge by finding a better continuous prompt. 

Besides, it is interesting to see a clear gap between BERT and GPT's improvement to the \solution. Fine-tuning with high-quality manual prompts (MP+FT)~\cite{schick2020small,gao2020making} has been proved to be quite effective, which is also observed in our experiments. However, it is surprising that GPTs do not benefit from MP+FT as much as from \solution as BERTs do. In other words, \solution shows a better affinity with unidirectional language models. In terms of much larger models such as MegatronLM\footnote{Provided in fairseq: \url{https://github.com/pytorch/fairseq/tree/master/examples/megatron_11b}} with 11 billion parameters, while fine-tuning hardly works, \solution is still applicable and achieve the state-of-the-art on LAMA.


























==> pt/pt_conclusion.tex <==
\section{Conclusion}

In this paper, we present--\textit{P-tuning}--which augments pre-trained model's ability in natural language understanding by automatically searching better prompts in the continuous space. 
Our \solution method relies less on a large validation set, suffers less from adversarial prompts, and alleviates over-fitting. 
We show that our \solution method can recover 64\% (P@1) of world knowledge from a pre-trained language model without any additional text provided during test time. On the SuperGLUE benchmark, \solution endows GPT-style models to show competitive performance with similar-size BERTs in natural language understanding, which is assumed impossible in the past. \solution also helps on bidirectional models and consequently outperforms state-of-the-art methods in the few-shot SuperGlue benchmark. It also proves that language models effectively capture more world knowledge and prior-task knowledge than we thought during pre-training.

==> pt/pt_exp.tex <==
\section{Experiments}
In this section, we conduct extensive experiments on two widely acknowledged natural language understanding benchmarks: LAMA~\cite{petroni2019language} knowledge probing and SuperGlue~\cite{wang2019superglue}. The encouraging results show that P-tuning can substantially boost GPTs' performance on natural language understanding, and BERT-style models can also be improved with a smaller gain.


\input{5_1_LAMA}










\begin{table*}[tb]
    \footnotesize
    \centering
    \begin{threeparttable}
    \begin{tabular}{l|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}}
    \toprule[1pt]
    \multirow{2}{*}{Method} & BoolQ & \multicolumn{2}{c|}{CB} & WiC & RTE & \multicolumn{2}{c|}{MultiRC}  & WSC & COPA & \multirow{2}{*}{Avg.} \\ 
    & (Acc.) & (Acc.) & (F1) & (Acc.) & (Acc.) & (EM) & (F1a) & (Acc.) & (Acc.) \\ 
    \hline
    \multicolumn{10}{c}{BERT-base-cased (109M)} \\
    \hline
    Fine-tuning & 72.9 &	85.1 & 73.9 & 71.1 & 68.4 & 16.2 & 66.3 & 63.5 & 67.0 
    & 66.2\\	
    MP zero-shot & 59.1 & 41.1 & 19.4 &  49.8 & 54.5 & 0.4 & 0.9 & 62.5 & 65.0 
    & 46.0\\
    MP fine-tuning & 73.7 & 87.5 & 90.8 & 67.9 & 70.4 & 13.7 & 62.5 & 60.6 & 70.0 
    & 67.1\\
    \solution & 73.9 & 89.2 & 92.1 & 68.8 & 71.1 & 14.8 & 63.3 & 63.5 & 72.0	& 68.4\\
    \midrule[1pt]
    \multicolumn{10}{c}{GPT2-base (117M)} \\
    \hline
    Fine-tune 
    & 71.2 
    & 78.6 
    & 55.8 
    & 65.5 
    & 67.8 
    & 17.4
    & 65.8 
    & 63.0 
    & 64.4 & 63.0\\
    MP zero-shot 
    & 61.3 
    & 44.6 
    & 33.3 
    & 54.1 
    & 49.5 
    & 2.2 
    & 23.8 
    & 62.5 
    & 58.0 & 48.2\\
    MP fine-tuning 
    & 74.8 
    & 87.5 
    & 88.1 
    & 68.0 
    & 70.0 
    & 23.5 
    & 69.7 
    & 66.3 
    & 78.0 & 70.2 \\
    \solution
        & 75.0 \tiny{\color{red}{(+1.1)}}
        & 91.1 \tiny{\color{red}{(+1.9)}}
        & 93.2 \tiny{\color{red}{(+1.1)}}
        & 68.3 \tiny{\color{blue}{(-2.8)}}
        & 70.8 \tiny{\color{blue}{(-0.3)}}
        & 23.5 \tiny{\color{red}{(+7.3)}}
        & 69.8 \tiny{\color{red}{(+3.5)}}
        & 63.5 \tiny{\color{red}{(+0.0)}}
        & 76.0 \tiny{\color{red}{(+4.0)}}
        & 70.4 \tiny{\color{red}{(+2.0)}}
        \\
    \bottomrule[1pt]
    \end{tabular}
    \end{threeparttable}
    \caption{Fully-supervised learning on SuperGLUE dev with base-scale models. MP refers to manual prompt. For a fair comparison, MP zero-shot and MP fine-tuning report results of a single pattern, while anchors for \solution are selected from the same prompt. Subscript in red represents advantages of GPT with \solution over the best results of BERT.
    }
    \label{tab:fully:bert-gpt-base}
\end{table*}



\begin{table*}[tb]
    \footnotesize
    \centering
    \begin{threeparttable}
    \begin{tabular}{l|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}}
    \toprule[1pt]
    \multirow{2}{*}{Method} & BoolQ & \multicolumn{2}{c|}{CB} & WiC & RTE & \multicolumn{2}{c|}{MultiRC}  & WSC & COPA &\multirow{2}{*}{Avg.} \\ 
    & (Acc.) & (F1) & (Acc.) & (Acc.) & (Acc.) & (EM) & (F1a) & (Acc.) & (Acc.) \\ 
    \hline
    \multicolumn{10}{c}{BERT-large-cased (335M)} \\
    \hline
    Fine-tune$^*$ 
    & 77.7 
    & 94.6 
    & 93.7 
    & 74.9 
    & 75.8 
    & 24.7 
    & 70.5 
    & 68.3 
    & 69.0  & 72.5 \\
    MP zero-shot 
    & 49.7 
    & 50.0 
    & 34.2 
    & 50.0 
    & 49.9 
    & 0.6 
    & 6.5 
    & 61.5 
    & 58.0 & 45.0\\
    MP fine-tuning
    & 77.2 
    & 91.1 
    & 93.5 
    & 70.5 
    & 73.6 
    & 17.7 
    & 67.0 
    & 80.8 
    & 75.0 & 73.1\\
    \solution 
    & 77.8	
    & 96.4 
    & 97.4 
    & 72.7 
    & 75.5 
    & 17.1 
    & 65.6 
    & 81.7 
    & 76.0 &74.6\\
    \midrule[1pt]
    \multicolumn{10}{c}{GPT2-medium (345M)} \\
    \hline
    Fine-tune 
    & 71.0 
    & 73.2 
    & 51.2 
    & 65.2 
    & 72.2 
    & 19.2 
    & 65.8 
    & 62.5 
    & 66.0 & 63.1\\
    MP zero-shot 
    & 56.3 
    & 44.6 
    & 26.6 
    & 54.1 
    & 51.3 
    & 2.2	
    & 32.5 
    & 63.5 
    & 53.0 &47.3\\
    MP fine-tuning
    & 78.3 
    & 96.4 
    & 97.4 
    & 70.4 
    & 72.6 
    & 32.1 
    & 74.4 
    & 73.0
    & 80.0  & 74.9 \\
    \solution
    & 78.9 \tiny{\color{red}{(+1.1)}}
    & 98.2 \tiny{\color{red}{(+1.8)}}
    & 98.7 \tiny{\color{red}{(+1.3)}}
    & 69.4 \tiny{\color{blue}{(-5.5)}}
    & 75.5 \tiny{\color{blue}{(-0.3)}}
    & 29.3 \tiny{\color{red}{(+4.6)}}
    & 74.2 \tiny{\color{red}{(+3.7)}}
    & 74.0 \tiny{\color{blue}{(-7.7)}}
    & 81.0 \tiny{\color{red}{(+5.0)}} 
    & 75.6 \tiny{\color{red}{(+1.0)}}\\
    \bottomrule[1pt]
    \end{tabular}
    \begin{tablenotes}
        \item[*] \small We report the same results taken from SuperGLUE~\cite{wang2019superglue}.
    \end{tablenotes}
    \end{threeparttable}
    \caption{Fully-supervised learning on SuperGLUE dev with large-scale models. MP refers to manual prompt. For fair comparison, MP zero-shot and MP fine-tuning report results of a single pattern, while anchors for \solution are selected from the same prompt. Subscripts in red represents improvements of GPT with \solution over the best results of BERT.
    }
    \label{tab:fully:bert-gpt-large}
\end{table*}


\subsection{SuperGLUE}

To evaluate \solution, we perform experiments on the SuperGLUE~\cite{SuperGLUE2019} benchmark. There are 8 natural language understanding (NLU) tasks in total, and we focus on 7 of them as~\cite{schick2020small}, since the other ReCoRD~\cite{ReCoRD2018} adopts no prompts, thus no \solution.
Tasks include question answering (BoolQ~\cite{BoolQ2019} \& MultiRC~\cite{MultiRC2018}), textual entailment (CB~\cite{de2019commitmentbank} \& RTE~\cite{RTE2005}), co-reference resolution (WiC~\cite{wic-paper}), causal reasoning (COPA~\cite{COPA2011}), and word sense disambiguation (WSC~\cite{WSC2012}).

For experimental settings, we consider both a fully-supervised setting and a few-shot setting. 
In the fully-supervised setting, we use the entire training sets ($\mathcal{D}_{train}$) and use development sets ($\mathcal{D}_{dev}$) for model selection and hyper-parameter tuning. 
For the few-shot setting, the few-shot version of SuperGLUE (also known as FewGlue)~\cite{schick2020small} is adopted.
FewGLUE is a subset of SuperGLUE, each task consisting of 32 train data ($\mathcal{D}_{train32}$) and an additional unlabeled set ($\mathcal{D}_{unlabeled}$) of different size ranging from 400 to 20000.
Different from previous work~\cite{schick2020small} which assumes no development sets and adopts fixed hyper-parameters according to empirical selection (which essentially overfits the test sets), we construct appropriate few-shot development sets (denoted as $\mathcal{D}_{dev32}$).
Since it has been proven that larger development sets confer additional significant advantages~\cite{gao2020making}, $\mathcal{D}_{dev32}$ is built by randomly selecting samples from unused training data and is strictly restricted to be no larger than the size of few-shot train sets.
We adopt the same evaluation metrics as~\cite{schick2020small}.


We reformulate NLU tasks into blank filling tasks.
Unlike~\cite{schick2020small} that use patterns with human hand-crafted prompts, \solution puts initial prompt embeddings in different positions within patterns and then fine-tunes the prompt embeddings together with the pretrained models.
For fully-supervised settings, we use the AdamW optimizer with a linearly decayed learning rate. 
We perform grid search of hyper-parameters and take the best combination on $\mathcal{D}_{dev}$ or $\mathcal{D}_{dev32}$. Specifically, we take learning rates from {1e-5, 2e-5, 3e-5} and batch sizes from {16, 32}.
For small datasets (COPA, WSC, CB, RTE), we fine-tune pretrained models for 20 epochs.  
For larger datasets (WiC, BoolQ, MultiRC), we reduce the number of training epochs to be 10 as the model converges earlier.
We evaluate the performance of every epoch.
We use early stopping to avoid overfitting to the training data. 
For few-shot learning, we use the same hyperparameters as~\cite{schick2020small} except extending fine-tuning steps to be 3500 (instead of 250 as~\cite{schick2020small}), since the fine-tuning of prompt embeddings requires even more steps.


\solution can be used on all unidirectional and bidirectional models.
We choose models with similar scales of total computes for a fair comparison, where we choose to compare BERT-base~\footnote{We use the cased version of BERT for comparison since the vocabulary of GPT2 is also cased.} with GPT2-base and compare BERT-large with GPT2-medium. 
Models like RoBERTa have a similar model size but was trained with much larger compute, which should be compared with larger-scale GPTs. This is left to future work.
Besides, for few-shot learning, we also experiment with albert-xxlarge-v2, which is proved to be the best-performed pretrained models for the few-shot setting in~\cite{schick2020small}.
For each pretrained model, we report the performance of standard finetuning (i.e., classification using [CLS] embeddings), PET finetuning~\cite{schick2020small}, PET zero-shot, and \solution.



\subsubsection{Fully-supervised Learning}

The main results are shown in Table~\ref{tab:fully:bert-gpt-base} and Table~\ref{tab:fully:bert-gpt-large}.
Firstly, for both bert-base-cased and bert-large-cased models, \solution outperforms all the other bert-based models on 5 out of 7 tasks.
Exceptions are WiC and MultiRC, where \solution performs a little bit worse than standard fine-tune.
Since both WiC and MultiRC have relatively large train sets, we conjecture this can be attributed to the fact that standard fine-tune could take even more advantages from a larger dataset than \solution.
On the contrary, \solution appears to be more beneficial in low-resource settings.
Similar observations are also shown in Section~\ref{sec:few-shot}.
Secondly, for both gpt2-base and gpt2-medium models, \solution achieves the most promising results among all gpt2-base models.
Above all, we can conclude that \solution can effectively boost the NLU performance of both bert-based and gpt-based models.

Besides, under the scale of base models, gpt2-base with \solution outperforms the best results of BERT-based models on 6 out of 7 tasks while achieving comparable results on WiC.
Comparing with BERT-large models, GPT2-medium with \solution shows advantages on 4 out of 7 tasks while being comparable on RTE and WSC tasks.
The only exception is the WiC task.
It is noticed that on the WiC task, standard fine-tune shows the best results on different models with different settings.
We speculate that it is because the word sense disambiguation task is not appropriate for prompt-based MLM prediction.
Above all, we conclude that with \solution, GPT2 achieves comparable and even better performance as BERT-based models.
The discovery subverts our common belief that bidirectional models (such as BERT) are always better at NLU tasks than unidirectional models (such as GPT2).







% \vpara{SOTA for SuperGLUE Few-shot.}
\begin{table*}[tb]
    \footnotesize
    \centering
    \begin{threeparttable}
    \begin{tabular}{c|l|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}|p{1cm}<{\centering}}
        \toprule[1pt]
        \multirow{2}{*}{Dev size} & \multirow{2}{*}{Method} & BoolQ & \multicolumn{2}{c|}{CB} & WiC & RTE & \multicolumn{2}{c|}{MultiRC}  & WSC & COPA \\ 
         &  & (Acc.) & (Acc.) & (F1) & (Acc.) & (Acc.) & (EM) & (F1a) & (Acc.) & (Acc.) \\ \hline
        \multirow{3}{*}{32} & PET$^*$    & 73.2\tiny{$\pm$3.1} & 82.9\tiny{$\pm$4.3} & 74.8\tiny{$\pm$9.2}  & 51.8\tiny{$\pm$2.7}  & 62.1\tiny{$\pm$5.3}  & 33.6\tiny{$\pm$3.2} & 74.5\tiny{$\pm$1.2}   & 79.8\tiny{$\pm$3.5}  & 85.3\tiny{$\pm$5.1} \\
         & PET best$^\dagger$ & 75.1 & 86.9 & 83.5 & 52.6 & 65.7 & 35.2 & 75.0 & 80.4 & 83.3 \\ 
         & P-tuning 
         & 77.8 \tiny{\color{red}{(+4.6)}}
         & 92.9 \tiny{\color{red}{(+10.0)}}
         & 92.3 \tiny{\color{red}{(+17.5)}}
         & 56.3 \tiny{\color{red}{(+4.5)}}
         & 76.5 \tiny{\color{red}{(+14.4)}}
         & 36.1 \tiny{\color{red}{(+2.5)}}
         & 75.0 \tiny{\color{red}{(+0.5)}}
         & 84.6 \tiny{\color{red}{(+4.8)}}
         & 87.0 \tiny{\color{red}{(+1.7)}}
         \\ 
         \midrule[1pt]
         \multirow{3}{*}{Full}& GPT-3 & 77.5 & 82.1 & 57.2 & 55.3 & 72.9 & 32.5 & 74.8 & 75.0 & 92.0 \\
         & PET$^\ddagger$   & 79.4 & 85.1 & 59.4 & 52.4 & 69.8 & 37.9 & 77.3 & 80.1 & 95.0 \\
         & iPET$^\mathsection$  & 80.6 & 92.9 & 92.4 & 52.2 & 74.0 & 33.0 & 74.0 & -    & - \\ \bottomrule[1pt]
    \end{tabular}
    \begin{tablenotes}
        \item[*] \small We report the average and standard deviation of each candidate prompt's average performance.
        \item[$\dagger$] \small We report the best performed prompt selected on \textit{full} dev dataset among all candidate prompts.
        \item[$\ddagger$] \small With additional ensemble and distillation.
        \item[$\mathsection$] \small With additional data augmentation, ensemble, distillation and self-training.
    \end{tablenotes}
    \end{threeparttable}
    \vspace{-5pt}
    \caption{Few-shot learning (32 train samples) on SuperGLUE dev. Previous few-shot learning approaches use the original full dev set ($\mathcal{D}_{dev}$) for validation, which does not make sense. We construct a new dev set ($\mathcal{D}_{dev32}$) with 32 unused samples from original training set. Under fair comparison, \solution significantly outperforms PET ($\mathcal{D}_{dev32}$) and PET best ($\mathcal{D}_{dev32}$) on all tasks. More interestingly, \solution even outperforms GPT-3, PET ($\mathcal{D}_{dev}$) and iPET ($\mathcal{D}_{dev}$) on 4 out of 7 tasks. Subscripts in red represents the improvements of \solution over PET($\mathcal{D}_{dev32}$).}
    \label{tab:fewshot:ultimate}
\end{table*}

\subsubsection{Few-shot Learning}\label{sec:few-shot}

\vpara{Sub-optimal and Sensitive Manual Prompts.}
Initially, PET/iPET~\cite{schick2020small} has achieved the state-of-the-arts on SuperGLUE few-shot learning tasks with several manually-written prompts, which are effective, but sub-optimal and labor-intensive.
For a comprehensive understanding of manual prompts, comparative experiments are first conducted.
Table~\ref{tab:fewshot:prompts} shows the results of using different manual prompts and \solution.
First,
results show that the few-shot performance has no obvious correlations with prompts' semantics, format, grammar. Prompts that humans consider reasonable is not necessarily effective for language models. 
Second, minor changes in manual prompts would cause substantial performance differences.
Pretrained language models are pretty sensitive to the choice of prompts.
We can conclude that manual handwriting prompts are more complicated than we thought.
Moreover, Table~\ref{tab:fewshot:prompts} also proves that it is impossible to find the best-performed manual prompts using $\mathcal{D}_{dev32}$. 
This indicates it is also challenging to pick the best manual prompts out in the few-shot setting.
In contrast, \solution appears promising in automatically searching better prompts with far fewer hand-crafts.

\begin{table*}% [ht]
    \footnotesize
    \centering
    \begin{tabular}{l|c|c}
        \toprule[1pt]
       Prompt & $\mathcal{D}_{dev}$ Acc. & $\mathcal{D}_{dev32}$ Acc. \\ 
       \hline
       Does [PRE] agree with [HYP]? [MASK]. & 57.16 & 53.12\\
       Does [HYP] agree with [PRE]? [MASK]. & 51.38 & 50.00\\
       Premise: [PRE] Hypothesis: [HYP] Answer: [MASK]. & 68.59 & 55.20\\
       \text{[PRE]} question: [HYP]. true or false? answer: [MASK]. & 70.15 & 53.12\\
       \solution &  76.45 &  56.25 \\
       \toprule[1pt]
    \end{tabular}
    \vspace{-10pt}
    \caption{Few-shot performance comparison of different manual prompts and tuned prompts on RTE tasks using albert-xxlarge-v2. Experiments use $\mathcal{D}_{dev32}$ for model selection and hyper-parameter tuning and evaluate on $\mathcal{D}_{dev}$. There's no obvious correlations between manual prompts and performance. Besides, $\mathcal{D}_{dev32}$ is not able to select the best manual prompts.}
    \label{tab:fewshot:prompts}
\end{table*}


\vpara{Updated SOTA for SuperGLUE Few-shot Learning.}
Table~\ref{tab:fewshot:ultimate} presents the latest state-of-the-art results for SuperGLUE few-shot learning, achieved by \solution.
We compared it with several baselines, including PET~\cite{schick2020small} and GPT-3~\cite{brown2020language}, which achieves previous SuperGLUE Few-shot SOTA.

It is worth noting that, aside from manual prompt fine-tuning, the original PET \cite{schick2020small} adopts multiple additional technologies, including data augmentation, ensemble, and distillation, to boost the performance.
Besides, it performs model selection and hyper-parameter tuning by over-fitting test sets.
To ensure a fair comparison,
PET is re-experimented under our $\mathcal{D}_{dev32}$ setting, removing all auxiliary technologies (data augmentation, ensemble, and distillation). 
Considering PET provides multiple manual prompts, both averaged performance, and the best-performed-prompt performance are reported.



Table~\ref{tab:fewshot:ultimate} illustrates that \solution consistently outperforms PET ($\mathcal{D}_{dev32}$) and PET-best ($\mathcal{D}_{dev32}$) with manual prompts on all tasks. The improvements of solution over PET ($\mathcal{D}_{dev32}$) are larger than the standard deviations over multiple patterns on 5 out of 7 tasks, proving that \solution can search far better prompts than manual ones and significantly improve few-shot task performance. On tasks including CB,WiC,RTE and WSC, \solution even outperforms PET/iPET ($\mathcal{D}_{dev}$), which adopt auxiliary technologies (data augmentation, ensemble and distillation).
Compared with GPT-3, with much larger scale than \solution (albert-xxlarge-v2), \solution outperforms on 6 out of 7 tasks.
Results demonstrate the advantages of \solution in few-shot NLU tasks.

%%% TODO add more analysis



\subsubsection{Finetuning v.s. MP Finetuning v.s. \solution}


Table~\ref{tab:fully:bert-gpt-base} and Table~\ref{tab:fully:bert-gpt-large} present results of three tuning-based paradigms for improving NLU performance.
We are particularly interested in how these tuning-based paradigms perform differently.
Overall, \solution outperforms fine-tuning and MP fine-tuning on average by around 2 points on BERT-based models and more than 5 points on GPT2-based models.
Specifically, though \solution achieves the best results on most of the tasks, fine-tuning can outperform on tasks (e.g., WiC) that are hard to formulate as cloze questions.
Comparing \solution and MP fine-tuning, \solution generally shows more advantages than MP fine-tuning on average, since it is tricky for MP fine-tuning to find good manual prompts. In contrast, \solution can always automatically search for better prompts.

As a new paradigm of tuning pretrained models, \solution could search over a vast prompt space while tuning pretrained models' parameters.
Results demonstrate its competitive potential in prompting larger-scale pre-trained models that are hard to fine-tune.

%First, PET outperforms Pure Fine-tuning (MLM) on average (by 15.6 points) as well as on each task, proving the effectiveness of using prompts.
%Second, PET shows advantages over Manual-prompt-based zero shot learning on average (by 16.1 points) as well as on each task, which proves fine-tuning is an effective way for few-shot learning.
%Comparing both Pure Fine-tuning methods, we can observe that generally directly fine-tuning masked language models performs better than directly fine-tuning as an classification task.
%This could because by transforming classification problem into close-question style makes it more efficient to make use of prior knowledge within language models.
%However, we also observe that such advantages decrease or even disappear when it comes to multi-token tasks (i.e., COPA \& WSC).
%Moreover, \solution outperforms iPET (generation 4) by 1.79 points on average.
%It proves that, \solution benefits more from language models by search in continuous space for better prompts and achieves stable improvements.








==> pt/pt_intro.tex <==
\section{Introduction}
Language model pre-training has been a successful approach for many natural language processing tasks \cite{brown2020language}. Evidences suggest that during the pre-training, not only do language models learn contextualized text representations, but also grammar~\cite{vig2019multiscale, clark2019does}, syntactic~\cite{hewitt2019structural}, commonsense~\cite{davison2019commonsense} and even world knowledge~\cite{petroni2019language,wang2020language}. 

According to the training objectives, pre-trained language models can be divided into three categories: \textbf{unidirectional language models} (e.g., GPT~\cite{radford2019language}) for natural language generation (NLG), \textbf{bidirectional language models} (e.g., BERT~\cite{devlin2018bert}) for natural language understanding (NLU) and \textbf{hybrid language models} (e.g., XLNet~\cite{yang2019xlnet}, UniLM~\cite{dong2019unified}) for combining the first two paradigms. For long, researchers have observed that GPT-style models perform poorly for NLU tasks with fine-tuning, and thus assumed that they are not suitable for language understanding in nature. 

The emerging GPT-3~\cite{brown2020language} and its particular performance on few-shot and zero-shot learning with handcrafted prompts has swept the machine learning community. Its success suggests that giant unidirectional language models together with appropriate manual prompt may work for natural language understanding. However, handcrafting a best-performing prompt is like finding a needle in a haystack, which often requires impractically large validation sets. In many cases, prompt engineering effectively means overfitting the test set. Besides, it is easy to create adversarial prompts that result in a substantial performance decrease. In light of these problems, recent works have focused on automatically searching discrete prompts~\cite{jiang2020can,shin2020autoprompt,reynolds2021prompt,gao2020making} and demonstrated their effectiveness. However, since neural networks are inherently continuous, discrete prompts can be sub-optimal.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/final.pdf}
    \vspace{-6mm}
    \caption{Average scores on 7 dev datasets of SuperGlue. GPTs can be better than similar-sized BERTs on NLU with P-tuning.}
    \label{fig:example}
    \vspace{-6mm}
\end{figure}
In this work, we propose a novel method-- P-tuning-- to automatically search prompts in the continuous space to bridge the gap between GPTs and NLU applications.\footnote{Codes will be at \url{https://github.com/THUDM/P-tuning}} \solution leverages few continuous free parameters to serve as prompts fed as the input to the pre-trained language models. We then optimize the continuous prompts using gradient descent as an alternative to discrete prompt searching. 

The simple \solution method brings substantial improvements to GPTs. We examine the \solution based GPTs on two NLU benchmarks: the LAMA~\cite{petroni2019language} knowledge probing and SuperGLUE~\cite{wang2019superglue}. In LAMA knowledge probing where model parameters are fixed, compared to original handcraft prompts, GPTs based on \solution show absolute gains of 26.2\%-41.1\% in Precision@1. The best one achieves 64.2\% in LAMA, which significantly surpasses the state-of-the-art 45.2\% prompt searching approach. In another NLU benchmark, SuperGlue, we jointly apply the \solution and fine-tuning in both few-shot and fully supervised scenarios. As a result, GPTs present a competitive performance to BERT models with the same scales, and for some datasets, GPTs even outperform BERTs. Further experiments demonstrate that BERT-style models can also benefit from \solution to some extent. We show that ALBERT with \solution substantially outperforms previous approaches and achieves new state-of-the-art results on the few-shot SuperGLUE benchmark.

Our discovery breaks the stereotype that GPTs can only generate but do not understand. It also suggests that language models contain much more world knowledge and prior task knowledge than we previously assumed. \solution also serves as a general method to tune pre-trained language models for the best downstream task performance. To sum up, we make the following contributions:

\begin{itemize}
    \item We show that GPTs can be as competitive as BERTs in natural language understanding (sometimes even better) with P-tuning, which can boost pre-trained language models' performance. This reveals that the potential of GPT-style architectures for natural language understanding has been under-estimated.
    \item We show that \solution is a general method to improve GPTs and BERTs in both few-shot and fully-supervised settings. Particularly, with P-tuning, our method outperforms state-of-the-art methods on LAMA knowledge probing and few-shot SuperGlue, which indicates that language models have grasped more world knowledge and prior-task knowledge during pre-training than we previously thought.
\end{itemize}

==> pt/pt_method.tex <==
\section{Method: P-tuning}
In this section, we present the implementation of P-tuning. Similar to discrete prompts, the P-tuning only applies non-invasive modification to the input. Nevertheless, the P-tuning replaces the input embeddings of pre-trained language models with its differential output embeddings.

\begin{figure*}
    \centering
    \includegraphics[width=17cm]{figs/PT.pdf}
    \caption{An example of prompt search for ``The capital of Britain is [MASK]''. Given the context (blue zone, ``Britain'') and target (red zone, ``[MASK]''), the orange zone refer to the prompt tokens. In (a), the prompt generator only receives discrete rewards; on the contrary, in (b) the pseudo prompts and prompt encoder can be optimized in a differentiable way. Sometimes, adding few task-related anchor tokens (such as ``capital'' in (b)) will bring further improvement.}
    \label{fig:framework}
\end{figure*}







\subsection{Architecture}
Given a pre-trained language model $\mathcal{M}$, a sequence of discrete input tokens $\mathbf{x}_{1:n}=\{x_0, x_1, ..., x_n\}$ will be mapped to input embeddings $\{\mathbf{e}(x_0), \mathbf{e}(x_1), ..., \mathbf{e}(x_n)\}$ by the pre-trained embedding layer $\mathbf{e}\in\mathcal{M}$. In a specific scenario, condition on the context $\mathbf{x}$, we often use the output embeddings of a set of target tokens $\mathbf{y}$ for downstream processing. For instance, in the pre-training, $\mathbf{x}$ refers to the unmasked tokens while $\mathbf{y}$ refers to the [MASK] ones; and in the sentence classification, $\mathbf{x}$ refers to the sentence tokens while $\mathbf{y}$ often refers to the [CLS].

The function of a prompt $\mathbf{p}$ is to organize context $\mathbf{x}$, target $\mathbf{y}$ and itself into a template $T$. For example, in the task of predicting a country's capital (LAMA-TREx P36), a template may be ``The capital of Britain is [MASK]." (see Figure \ref{fig:framework}), in which ``The capital of ... is ... ." is prompt, ``Britain" is the context and ``[MASK]" is the target. Prompts can be so flexible that we may even insert them into the context or target.

Let $\mathcal{V}$ refers to the vocabulary of a language model $\mathcal{M}$ and [$\mathrm{P}_i$] refers to the $i^{\mathrm{th}}$ prompt token in a template $T$. For simplicity, given a template $T=\{[\mathrm{P}_{0:i}],\mathbf{x},[\mathrm{P}_{i+1:m}],\mathbf{y}\}$, compared to traditional discrete prompts which satisfy $[\mathrm{P}_i]\in\mathcal{V}$ and map the $T$ into
\begin{equation}
    \{\mathbf{e}([\mathrm{P}_{0:i}]), \mathbf{e}(\mathbf{x}),\mathbf{e}([\mathrm{P}_{i+1:m}]), \mathbf{e}(\mathbf{y})\}
\end{equation}
\solution instead regards the [$\mathrm{P}_i$] as pseudo tokens and map the template to
\begin{equation}
    \{h_0,...,h_i, \mathbf{e}(\mathbf{x}),h_{i+1},...,h_m, \mathbf{e}(\mathbf{y})\}
\end{equation}
where $h_i (0\leq i<m)$ are trainable embedding tensors. This enables us to find a better continuous prompts beyond the original vocabulary $\mathcal{V}$ of $\mathcal{M}$ could express. Finally, with the downstream loss function $\mathcal{L}$, we can differentially optimize the continuous prompt $h_i (0\leq i<m)$ by
\begin{equation}
    \hat{h}_{0:m}=\mathop{\arg\min}_h\mathcal{L}(\mathcal{M}(\mathbf{x}, \mathbf{y}))
\end{equation}







\subsection{Optimization}
Although the idea of training continuous prompts is straightforward, in practice, it faces two optimization challenges: 1) \textbf{Discreteness:} the original word embedding $\mathbf{e}$ of $\mathcal{M}$ has already become highly discrete after pre-training. If $h$ is initialized with random distribution and then optimized with stochastic gradient descent (SGD), which has been proved to only change the parameters in a small neighborhood~\cite{allen2019convergence}, the optimizer would easily fall into local minima. 2) \textbf{Association:} another concern would be, intuitively, we believe the values of prompt embeddings $h_i$ should be dependent on each other rather than independent. We need some mechanism to associate prompt embeddings with each other.

In light of the challenges, in the \solution we propose to also model the $h_i$ as a sequence using a prompt encoder consists of a very lite neural network that can solve the discreteness and association problems. And in practice, we choose a bidirectional long-short term memory networks (LSTM), with a ReLU activated two-layer multilayer perceptron (MLP) to encourage discreteness. Formally speaking, the real input embeddings $h^\prime_i$ to the language model $\mathcal{M}$ is derived from
\begin{equation}
\begin{split}
    h_i &= \mathrm{MLP}([\overrightarrow{h_i}:\overleftarrow{h_i}])\\
    &=\mathrm{MLP}([\mathrm{LSTM}(h_{0:i}):\mathrm{LSTM}(h_{i:m})])
\end{split}
\end{equation}

Though the LSTM head's use indeed adds some parameters to the training of continuous prompts, the LSTM head is several magnitude orders smaller than the pre-trained model. Moreover, in the inference, we only need the output embedding $h$ and can discard the LSTM head.

Besides, we also find that adding few anchor tokens helps some NLU tasks in the SuperGLUE benchmark. For instance, for RTE task, the token ``?'' within prompt template ``[PRE][prompt tokens][HYP]?[prompt tokens][MASK]'' is specially added as an anchor token and affects the performance a lot. Usually such anchor words characterize each component, where in this case ``?'' indicate that ``[HYP]'' acts as an interrogation part.


























==> pt/pt_motivation.tex <==
\section{Motivation}
The miracle of GPT-3~\cite{brown2020language} and DALL-E~\cite{ramesh2021zero} seem to suggest that giant models are always nothing short of a panacea for boosting machine intelligence. However, behind the prosperity, there are unignorable challenges. 

A fatal one is that giant models suffer from poor transferability. Fine-tuning on downstream tasks hardly works for those trillion-scale models. Even for the many-shot fine-tuning setting, these models are still too large to memorize the fine-tuning samples~\cite{yue2020interventional} quickly. 

As a substitution, GPT-3 and DALL-E have been reported to leverage handcrafted prompts to steer the model for downstream applications. However, handcraft prompt searching heavily relies on impractically large validations sets, but its performance is also volatile. We show a similar case in LAMA~\cite{petroni2019language} knowledge probing (Table \ref{tab:motivation_lama}), where a single-word's change can cause a drastic difference. 

\begin{table}[h]
    \small
    \centering
    \begin{tabular}{l|c}
       \toprule[1pt]
       Prompt & P@1 \\ \hline
       [X] is located in [Y]. \textit{(original)} & 31.29 \\ \hline
       [X] is located in which country or state? [Y]. & 19.78 \\ \hline
       [X] is located in which country? [Y]. & 31.40 \\ \hline
       [X] is located in which country? In [Y]. & 51.08 \\ 
       \toprule[1pt]
    \end{tabular}
    \caption{Case study on LAMA-TREx P17 with bert-base-cased. A single-word change in prompts could yield a drastic difference.}
    \label{tab:motivation_lama}
\end{table}

In light of the challenge, while some recent works have concentrated on automating the search of discrete prompts by mining training corpus~\cite{jiang2020can}, gradient searching~\cite{shin2020autoprompt} and using separate model~\cite{gao2020making}, we delve into the problem of finding continuous prompts that can be differentially optimized.

==> pt/pt_unused_problem.tex <==
\section{Problem Setup}

Language models could grasp knowledge during pre-training from scratch, but it is difficult to evaluate. Although super large language models keep breaking records in wide range of downstream tasks, the fact that it requires sufficient fine-tuning confuses the knowledge learned during the pre-training with what is learned during the fine-tuning, and thus fails to demonstrate what language models really learn much knowledge from pre-training.

To evaluate the authentic knowledge language models acquired from pre-training, in this work we propose two proxy tasks that require no or minimum efforts for fine-tuning: knowledge probing and few-shot learning.

\subsection{Knowledge Probing}
Narrowly speaking, the knowledge usually refers to the world knowledge in the knowledge base. The knowledge probing, or mentioned as fact retrieval, is about evaluating how much real-world knowledge has language models gained from pre-training. The LAMA dataset evaluates it with cloze tests created from triples selected in the knowledge bases. For example, we will transform the triple (Dante, born-in, Florence) into a cloze sentence with handcraft prompt ``Dante was born in [MASK].", and then we ask language models to perform zero-shot inference.

\subsection{Few-shot Learning}


In addition to world knowledge, it has been proved that language models can also provide prior knowledge for specific downstream tasks (denoted as prior-task knowledge).
The commonly-used few-shot learning tasks are considered.
By using prompts to reformulate inputs into cloze-style phrases and equally transform the discriminative few-shot tasks into masked language model tasks, they are able to make use of the linguistic knowledge within language model.
For example, a sentiment analysis task (``Best movie ever!'', +1) would be transformed into masked language model tasks (``Best movie ever! It was [MASK].''), where predicting ``[MASK]'' to be ``great'' equals ``+1'' labeling.
In this way, the inherent linguistic knowledge would guide the prediction of masked token, which further help few-shot task prediction.


Similar to knowledge probing, the prompt-based prediction can be directly performed over given pretrained language models in a zero-shot manner.
Particularly, since different tasks are independent, it is also applicable for few-shot learning to fine-tune on given pretrained language models, making them more adaptive for specific tasks.




